Thinking Hard, Not Smart: Reasoning Models Fail to Ration Test-Time Compute Across Questions

Reasoning language models increasingly use test-time compute to improve performance, but existing evaluations typically study this compute one question at a time. Yet when multiple problems share an end-to-end cost or latency constraint, models must decide how to divide limited inference compute among them. We introduce an exam-style evaluation framework for studying this setting, in which a model must distribute one shared token budget across questions with different difficulty and point values to maximize its total score. Across several open and frontier reasoning models, we find that models fail to allocate a shared budget strategically across questions of varying difficulties and values. Models behave largely as greedy sequential solvers: they prioritize questions by presentation order, front-load effort on early questions, and remain insensitive to value, with these tendencies becoming more pronounced as the number of questions grows. Explicit planning prompts spread compute more evenly but do not produce value- or difficulty-aware prioritization. The same behavioral pattern extends from mathematical to code reasoning. These findings establish global budget allocation as a distinct capability that is not captured by conventional per-question evaluation and remains a challenge for current reasoning models.

==> archive_v1/img_tab_tex/LLM_judge_prompt.tex <==
\begin{figure*}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\linewidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Instruction to the LLM Judge},
  fonttitle=\bfseries,
  % fontupper=\ttfamily
]
You are an expert mathematics judge. Your task is to evaluate whether the model's answers match the reference answers for a set of math questions. The reference answers are always correct, and the model's answers may be correct, incorrect, or incomplete.
\\

\{original\_questions\_text\}

\{ref\_text\}

\{model\_text\}

\{score\_text\}
\\

Please evaluate each answer for correctness. Consider the following:
1. Mathematical equivalence (e.g., 0.25 == 1/4, sqrt(3) == $\sqrt{3}$)
2. Different forms of the same answer (e.g., simplified vs expanded forms)
3. LaTeX formatting differences should not affect correctness
\\

For each question, award the full points if the answer is correct, and 0 points if incorrect.
\\

Provide your evaluation in the following JSON format:

\begin{verbatim}
{{
    "evaluations": [
        {{
            "question": 1,
            "correct": true/false,
            "score_awarded": <points>,
            "explanation": "<brief explanation>"
        }},
        ...
    ],
    "total_score": <sum of all awarded scores>,
    "max_score": <sum of all possible scores>
}}
\end{verbatim}

Respond with ONLY the JSON, no additional text.

\end{tcolorbox}
\caption{The instruction to \texttt{GPT-5} for it to serve as an LLM-as-a-judge.}
\label{fig:judge_prompt}
\end{figure*}

==> archive_v1/img_tab_tex/baseline_orderings.tex <==
\begin{table*}[ht]
\centering

\footnotesize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}l*{9}{c}@{}}
\toprule
\textbf{Model}
  & \multicolumn{3}{c}{\textbf{5 Qs}}
  & \multicolumn{3}{c}{\textbf{10 Qs}}
  & \multicolumn{3}{c}{\textbf{20 Qs}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
 & \textbf{rand.} & \textbf{e$\rightarrow$h} & \textbf{h$\rightarrow$e}
 & \textbf{rand.} & \textbf{e$\rightarrow$h} & \textbf{h$\rightarrow$e}
 & \textbf{rand.} & \textbf{e$\rightarrow$h} & \textbf{h$\rightarrow$e} \\
\midrule
Qwen3-14B      & 25.9 & 24.6 & 21.4 & 17.2 & 15.3 & 13.6 &  7.6 & 11.6 & 10.8 \\
Qwen3-8B       & 13.7 & 12.8 & 17.9 &  8.8 &  8.6 &  7.6 &  7.5 &  7.0 &  5.2 \\
DS-R1-Llama-8B & 13.8 & 16.9 & 14.3 &  9.1 & 10.1 &  8.6 &  5.1 &  6.1 &  5.5 \\
DS-R1-Qwen-14B & 22.4 & 24.0 & 31.3 & 17.2 & 17.2 & 16.0 & 14.0 &  9.0 &  9.8 \\
DS-R1-Qwen-7B  & 10.6 & 13.1 & 15.6 &  7.7 &  5.6 &  3.3 &  3.1 &  3.0 &  2.1 \\
Llama-3.1-8B   &  7.8 &  5.5 &  3.9 &  7.2 &  5.5 &  2.8 &  3.3 &  4.3 &  3.3 \\
\bottomrule
\end{tabular}
\caption{Score rates (\%) under a fixed 10K token budget with no explicit guidance regarding budget allocation, shown separately for different question orderings. Within each question-count block, the 3 columns corresponds to random ordering (rand.), increasing difficulty (e$\rightarrow$h), and decreasing difficulty (h$\rightarrow$e). Overall, performance degrades as question count increases, larger models consistently outperform smaller ones, and question ordering has negligible impact, highlighting limitations in adaptive budget allocation.}
\label{tab:baseline}
\end{table*}


==> archive_v1/img_tab_tex/combined_difficulty_based.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/combined_grouped_stacked_plot_difficulty_based.pdf}
    \caption{Score rates under difficulty-proportional scoring. Rows show question ordering, model panels are separated by dashed lines, and bars compare strategy conditions across 5, 10, and 20-question exams. Red bars denote the uniform-allocation baseline, which splits the global budget evenly across questions and aggregates the resulting exam score. Overall, human-like test-taking strategies provide modest but nontrivial gains in some settings, longer exams are consistently harder to solve under a shared reasoning budget, but question ordering has a weak and model-dependent effect. Many model dynamic budget allocations fail to beat the uniform allocation baselines.}
    \label{fig:difficulty-proportional-results}
\end{figure*}


==> archive_v1/img_tab_tex/combined_fixed.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/combined_grouped_stacked_plot_fixed.pdf}
    \caption{Score rates under fixed scoring, where all questions receive equal point values. The red uniform-allocation baseline evenly splits the global budget across questions. This setting removes point-value variation, isolating budget management across equally rewarded questions. The same exam-length degradation and uniform-baseline underperformance persist even without score-based prioritization.}
    \label{fig:fixed-score-results}
\end{figure*}


==> archive_v1/img_tab_tex/explicit_plan_prompt.tex <==
\begin{figure}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\linewidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Prompt for Explicit Planning},
  fonttitle=\bfseries,
  % fontupper=\ttfamily
]
Each question has a different difficulty and may require a different amount of reasoning to answer correctly. You should plan your allocation/spending wisely to maximize the total score.


\end{tcolorbox}
\end{figure}

==> archive_v1/img_tab_tex/full_QA_prompt.tex <==

\begin{figure*}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\textwidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Prompt to the LLM During Inference},
  fonttitle=\bfseries,
]
Below is a list of questions that you need to answer. Each question has an associated score (as shown in ``This question is worth ...'') and your goal is to maximize the total score obtained. For each question, you get full score if you answer it correctly, and zero if you answer it incorrectly. You in total have a reasoning budget of \emph{budget} tokens.

\medskip
\textbf{Optional strategy hints used in some conditions.} We additionally include one or more of the following sentences depending on the experimental setting:
\begin{itemize}[leftmargin=12pt]
    \item \emph{Explicit plan:} ``Each question has a different difficulty and may require a different amount of reasoning to answer correctly. You should plan your allocation/spending wisely to maximize the total score.''
    \item \emph{Skip hint:} ``You may even choose to not answer some questions if you think the cost of answering them is too high compared to the potential score gain.''
    \item \emph{Recheck hint:} ``If you think you have more than enough budget, you may also recheck and refine your answers to early questions to further increase the chances of maximizing the total score, but keep in mind that the rechecking also consumes your reasoning budget.''
\end{itemize}

\medskip
Questions:
\begin{verbatim}
Q1: [question text] (This question is worth [score] points)
Q2: [question text] (This question is worth [score] points)
...
QN: [question text] (This question is worth [score] points)
\end{verbatim}

Think through each question carefully to maximize your total score. Begin your reasoning now.
\end{tcolorbox}
\caption{The prompt used during inference. The exact wording varies slightly depending on the experimental condition through optional strategy hints.}
\label{fig:inference_prompt}
\end{figure*}

==> archive_v1/img_tab_tex/recheck_answer_prompt.tex <==
\begin{figure}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\linewidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Prompt for Rechecking Answers},
  fonttitle=\bfseries,
  % fontupper=\ttfamily
]
If you think you have more than enough budget, you may also recheck and refine your answers to early questions to further increase the chances of maximizing the total score, but keep in mind that the rechecking also consumes your output budget.


\end{tcolorbox}
\end{figure}

==> archive_v1/img_tab_tex/skip_question_prompt.tex <==
\begin{figure}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\linewidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Prompt for Question Skipping},
  fonttitle=\bfseries,
  % fontupper=\ttfamily
]
You may even choose to not answer some questions if you think the cost of answering them is too high compared to the potential score gain.


\end{tcolorbox}
\end{figure}

==> archive_v1/img_tab_tex/teaser_fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/project_teaser_figure_saved.pdf}
    \caption{\textbf{A comparison between standard evaluation, budget-constrained evaluation, and our exam-style evaluation.} In standard evaluation, models answer one question at a time with an unrestricted token budget. Budget-constrained evaluation limits tokens per question. In our exam-style evaluation, a fixed total budget is given for a set of problems with varying scores and difficulties, testing a model’s ability to allocate resources strategically under constraints.}
    \label{fig:teaser}
\end{figure}

==> archive_v1/sec/conclusion.tex <==
\section{Conclusion}

We introduced an exam-style evaluation framework for measuring whether LLMs can allocate a fixed reasoning budget across multiple questions to maximize total score. Unlike standard single-question evaluation, this setting tests cross-question planning, prioritization, and budget control under a shared compute constraint. On Omni-MATH exam instances, we find that longer exams substantially reduce score rate, human-like strategy prompts provide modest but inconsistent gains, and question ordering has weak and model-dependent effects. Most importantly, several global-budget prompting settings underperform a naive uniform-allocation baseline, especially for smaller models and longer exams. These results suggest that current reasoning models do not yet reliably manage a shared reasoning budget, even when they are explicitly instructed to do so. Extending this framework beyond mathematics to domains such as multi-hop question answering, code, and tool-using agents is an important next step.


==> archive_v1/sec/exp.tex <==
\section{Experiments}
 
\paragraph{Benchmark and models.}
 
We construct exam-style evaluation sets by randomly sampling and concatenating problems from Omni-MATH~\citep{gao2024omnimathuniversalolympiadlevel}, an olympiad-level mathematical reasoning benchmark. Each evaluation instance consists of a set of $N$ questions bundled into a single prompt, where $N \in \{5, 10, 20\}$. This range is chosen to simulate exams of varying length and to test how models cope with increasing numbers of competing questions under a shared budget. Each question is assigned a point value and a difficulty label drawn from the original benchmark metadata.
 
We evaluate six open-weight language models spanning two parameter scales: four 7--8B models (Llama-3.1-8B-Instruct~\citep{grattafiori2024llama}, DeepSeek-R1-Distill-Qwen-7B, DeepSeek-R1-Distill-Llama-8B~\citep{guo2025deepseek}, and Qwen3-8B~\citep{yang2025qwen3}) and two 14B models (DeepSeek-R1-Distill-Qwen-14B~\citep{guo2025deepseek} and Qwen3-14B~\citep{yang2025qwen3}).
 
All models are served locally using vLLM~\citep{kwon2025vllm} with a fixed output token budget of 10{,}000 tokens.
 
\paragraph{Question Ordering}
 
To investigate whether the presentation order of questions affects a model's allocation strategy, we evaluate each model under three orderings:
\begin{itemize}
    \item \textbf{As-is (\texttt{asis})}: The original order from the sampled question set.
    \item \textbf{Ascending difficulty (\texttt{difficulty\_asc})}: Questions sorted from easiest to hardest.
    \item \textbf{Descending difficulty (\texttt{difficulty\_desc})}: Questions sorted from hardest to easiest.
\end{itemize}
 
\paragraph{Prompting Strategy (Baseline)}
 
In the baseline setting (\texttt{one\_round\_baseline}), the model receives a single prompt containing all $N$ questions along with an instruction specifying the total token budget. No additional guidance is provided regarding how to plan, prioritize, or skip questions. This serves as the control condition against which more elaborate prompting strategies are compared.
 
\paragraph{Evaluation}
 
Model outputs are evaluated using GPT as a judge model. For each question, the judge compares the model's answer against the reference solution and assigns a binary correctness label. We report two metrics:
\begin{itemize}
    \item \textbf{Accuracy (score rate)}: The fraction of total available points earned by correctly answered questions.
    \item \textbf{Budget compliance}: The fraction of evaluation instances in which the model's output stays within the 10{,}000-token budget.
\end{itemize}
 
% ============================================================
 
\subsection{Results}
\label{sec:baseline}
 
Table~\ref{tab:baseline} summarizes the accuracy of all six models under the baseline prompting strategy across three question set sizes and three question orderings.

 
 
Several trends emerge from the baseline results. Accuracy degrades sharply as the number of questions grows, with all models showing a substantial drop from 5 to 20 questions, confirming that distributing a fixed budget across more problems is the central challenge. The two 14B models consistently outperform all 7--8B models by a clear margin across every setting. Budget compliance is nearly zero for all models except Llama-3.1-8B-Instruct, which achieves 24--45\% compliance but at the cost of the lowest accuracy, suggesting a trade-off between respecting the budget and producing substantive reasoning. Question ordering (\texttt{asis}, \texttt{difficulty\_asc}, \texttt{difficulty\_desc}) has no consistent effect on performance, indicating that models do not adapt their allocation strategy to the difficulty progression under the baseline prompt.




==> archive_v1/sec/intro.tex <==
\section{Introduction}


Large language models (LLMs) have achieved remarkable progress in complex reasoning tasks~\cite{wei2023chainofthoughtpromptingelicitsreasoning, jaech2024openai, Guo_2025, muennighoff2025s1}. By scaling inference-time computation and producing extended reasoning traces, modern models now rival or even surpass human performance across a wide range of domains. For example, LLMs exceed 95\% accuracy on grade-school mathematics benchmarks~\citep{cobbe2021trainingverifierssolvemath}, and recent models such as GPT-5~\citep{openai2025gpt5} and Gemini-2.5-Pro~\citep{comanici2025gemini25pushingfrontier} outperform top 1\% human participants on competition-level mathematics~\citep{balunović2026matharenaevaluatingllmsuncontaminated} while achieving PhD-level performance on specialized question sets~\cite{rein2023gpqagraduatelevelgoogleproofqa}.


\input{img_tab_tex/teaser_fig}

However, a fundamental mismatch remains between how humans and LLMs are typically evaluated. Human examinations are designed as time-limited, multi-question assessments that require test-takers to distribute effort across problems with different difficulty levels and point values. Performance therefore depends not only on solving individual questions correctly, but also on making strategic decisions about when to spend more time, when to skip, and when to revisit an answer. In contrast, current LLM benchmarks usually evaluate models one question at a time and often permit unrestricted reasoning per instance without budget constraints (Figure~\ref{fig:teaser}(a))~\cite{cobbe2021trainingverifierssolvemath,rein2023gpqagraduatelevelgoogleproofqa,gao2024omnimathuniversalolympiadlevel}. Even in efficiency-aware and budget-constrained evaluations, constraints are usually imposed at the per-question level~\cite{ma2025reasoningmodelseffectivethinking, wen2025budgetthinkerempoweringbudgetawarellm}, rather than across a set of tasks. As a result, current evaluations fail to capture a model’s ability to strategically plan and allocate resources across multiple problems.

This missing dimension matters for two reasons. First, inference-time computation is not free. In practical deployments, reasoning tokens translate into latency, monetary cost, energy use, and limited context capacity. An agent may need to solve many subtasks in a single interaction, triage a batch of user requests, or make progress when external tools and retrieval are unavailable or too costly. In these settings, the central question is not only whether the model can eventually solve each isolated problem, but whether it can spend a fixed computational budget where it yields the highest return. A model that overthinks early or low-value subtasks can fail even if it is individually capable on the underlying questions.

Second, budget-constrained evaluation may be more informative about a model's reasoning competence. In human assessment, intelligence is not only reflected in knowing an answer after unlimited time, but also in recognizing what needs to be solved, what can be answered quickly, and what should be deferred under limited time. This ability to decide what information is worth acquiring or verifying is itself a form of strategic cognition. We therefore view global-budget evaluation as a way to probe whether LLMs possess not just local problem-solving skill, but also the meta-level judgment needed to allocate reasoning effort across competing objectives.

To bridge this gap, we propose evaluating LLMs under exam-like conditions (Figure~\ref{fig:teaser}(c)): Given a fixed total token budget, a model must complete a set of tasks with varying difficulty and points and is scored by its total accumulated points. This formulation more closely mirrors human test-taking and explicitly evaluates strategic reasoning under limited resources. Moreover, prior work in educational measurement and psychometrics~\cite{goldhammer2015measuring,vanderlinden2007hierarchical} shows that timed tests reveal additional information about ability and cognitive processing. We hypothesize that the same principle would also apply to LLMs, making budget-constrained, multi-question evaluation more discriminative than conventional single-question settings.



Together, these motivations connect benchmark design with practical agent behavior: global-budget evaluation lets us test whether a model can turn strong local reasoning ability into effective resource allocation across competing objectives. Our exam-style framework provides a controlled and practical way to evaluate, and ultimately improve, this capability.

Our findings show that under exam-style evaluation, human-like test-taking strategies provide modest but nontrivial gains in some settings, longer exams are consistently harder to solve under a shared reasoning budget, and question ordering has a weak and model-dependent effect across scoring schemes. Moreover, many settings fail to outperform a naive uniform-allocation baseline, especially for smaller reasoning models and longer exams, suggesting that current models do not reliably translate a global budget instruction into effective cross-question planning.


% \Chenrui{Efficiency and overthinking?}


% [Why we do this]
% (1) A fair comparison with human
% (2) Such testing format might be better to distinguish 'better' model 
% (3) Potential application scenarios: [1] LLM batch process. [2] Agent decompose a complex task, plan and execute steps.


==> archive_v1/sec/method.tex <==
% \section{Method}
% We evaluate the capability of Large Language Models (LLMs) to strategically allocate a limited budget across multiple problems to maximize overall performance. We formulate this evaluation by presenting the model with a concatenated list of questions in a single prompt, where each question varies in difficulty and point value. To comprehensively assess the model's resource allocation strategies, our evaluation encompasses three key dimensions.

% \paragraph{Score assignment strategies.}
% To simulate human exam conditions, each question is assigned a point value. We examine both difficulty-independent and difficulty-dependent scoring methods:
% \begin{itemize}
%     \item \textbf{Difficulty-independent scoring:} We test \textit{random scoring}, where each question is assigned a random value between 1 and 15, and \textit{fixed scoring}, where all questions are uniformly worth 10 points regardless of difficulty.
%     \item \textbf{Difficulty-dependent scoring:} We test scoring that is \textit{proportional to difficulty} (harder questions yield higher scores) and \textit{inversely proportional to difficulty} (harder questions yield lower scores). The inversely proportional setting is specifically designed to test the model's ability to balance risk and reliable returns. It evaluates whether the model recognizes that spending a large portion of its budget on a difficult question yields a minimal reward, penalizing it for missing easier, higher-yield questions due to a depleted budget.
% \end{itemize}

% \paragraph{Question ordering.}
% Just as the sequence of questions can significantly impact a human test-taker's performance \cite{}, it may also influence LLM resource allocation. We evaluate three ordering configurations:
% \begin{itemize}
%     \item \textbf{Increasing difficulty:} Mirrors traditional exams, starting with the easiest questions and progressively getting harder.
%     \item \textbf{Decreasing difficulty:} The reverse order, front-loading the most difficult questions.
%     \item \textbf{Random ordering:} Questions are shuffled independently of their difficulty levels.
% \end{itemize}

% \paragraph{Explicit vs. implicit planning.}
% Finally, we investigate the impact of prompting the model to explicitly plan its budget allocation before attempting the questions. In the \textit{implicit planning} (without explicit planning) setup, we evaluate whether the model innately possesses global-goal awareness. This tests if the model can internally weigh question difficulties and autonomously manage its budget to maximize its completion rate without step-by-step guidance.



\section{Exam-style Evaluation for LLMs}
We evaluate whether LLMs can strategically allocate a limited budget across multiple questions to maximize total score. An exam instance is a set of questions $\mathcal{E}=\{(q_i,s_i)\}_{i=1}^{N}$, where $q_i$ is a question and $s_i$ is its point value. The model receives all questions in one prompt and a single global reasoning budget $B$ measured in output tokens. Its objective is to produce answers $\{a_i\}_{i=1}^{N}$ that maximize
\begin{equation}
    \sum_{i=1}^{N} s_i \cdot \mathbf{1}\{\mathrm{Judge}(q_i,a_i)=1\},
\end{equation}
subject to using at most $B$ reasoning tokens before final answers are forced. Thus, the budget is the total amount of reasoning computation available for the whole exam, and the score is the task utility obtained under that fixed compute constraint. In Section~\ref{sec:setup}, we explain the detailed setup regarding data, models, inference, budget forcing, and performance measurement. We then introduce two ablative dimensions: exam design choices in Section~\ref{sec:exam-design-choice} and human test-taking strategies in Section~\ref{sec:test-taking-strategy}. The results and analysis are in Section~\ref{sec:results}.

% \subsection{Setup}
% \paragraph{Dataset.} 
% We construct exam-style evaluation sets by randomly sampling and concatenating problems from Omni-MATH~\citep{gao2024omnimathuniversalolympiadlevel}, an olympiad-level mathematical reasoning benchmark. Each evaluation instance consists of a set of $N$ questions bundled into a single prompt, where $N \in \{5, 10, 20\}$. This range is chosen to simulate exams of varying lengths and to test how models cope with increasing numbers of questions under a shared budget. Each question has a corresponding difficulty label drawn from the original benchmark metadata, but the difficulty label is not directly exposed to the model.

% \paragraph{Models and Sampling Parameters.}
% We evaluate six open-weight language models spanning two parameter scales: four 7--8B models (Llama-3.1-8B-Instruct~\citep{grattafiori2024llama}, DeepSeek-R1-Distill-Qwen-7B, DeepSeek-R1-Distill-Llama-8B~\citep{guo2025deepseek}, and Qwen3-8B~\citep{yang2025qwen3}) and two 14B models (DeepSeek-R1-Distill-Qwen-14B~\citep{guo2025deepseek} and Qwen3-14B~\citep{yang2025qwen3}). All inference runs use \texttt{Temperature}=0.6, \texttt{TopP}=0.95, and \texttt{TopK}=20. 



% \paragraph{Budget.} For each evaluation instance, regardless of the value of $N$, the model is given a total budget of 20,000 tokens. If the model has not finished its response after the budget is reached, we forcefully truncate the output and append ``So the final answer is:'' to force the model to give its final answer, similar as how a human test taker would do in desperate when the exam time is up. 



% \paragraph{Evaluation and Metrics.} The correctness of model responses on the evaluation instances are judged by LLM-as-a-judge using \texttt{GPT-5}~\cite{openai2025gpt5}. The detailed judge instruction is shown in Figure~\ref{append:llm_judge_prompt}. Performance is measured by score rate (\%), defined as \begin{equation}
%     \text{Score Rate}=\frac{\text{Achieved score}}{\text{Max achievable score}}.
% \end{equation}
% For each question, the model receives full score if the answer is correct, and zero score otherwise. The max achievable score is the sum of the assigned scores for all questions within one evaluation instance.

\subsection{Setup}
\label{sec:setup}
\paragraph{Dataset.} 
We construct exam-style evaluation sets by randomly sampling and concatenating problems from Omni-MATH~\citep{gao2024omnimathuniversalolympiadlevel}, an olympiad-level mathematical reasoning benchmark. We use mathematics as a controlled first testbed because it provides answer-verifiable tasks, meaningful difficulty variation, and reasoning traces whose token cost can vary substantially across questions. Each evaluation instance consists of a set of $N$ questions bundled into a single prompt, where $N \in \{5, 10, 20\}$. This range is chosen to simulate exams of varying lengths and to test how models cope with increasing numbers of questions under a shared budget. Each question has a corresponding difficulty label drawn from the original benchmark metadata, but the difficulty label is not directly exposed to the model. While multi-hop question answering, code, and tool-use tasks are also natural domains for exam-style evaluation, we leave them to future work and focus here on isolating budget allocation in a clean mathematical setting.

\paragraph{Models and Sampling Parameters.}
We evaluate four open-weight reasoning models: DeepSeek-R1-Distill-Qwen-7B and DeepSeek-R1-Distill-Qwen-14B~\citep{guo2025deepseek}, as well as Qwen3-8B and Qwen3-14B~\citep{yang2025qwen3}. In the reasoning phase, all inference runs use \texttt{Temperature}=0.6, \texttt{TopP}=0.95, and \texttt{TopK}=20.

\paragraph{Prompting.}
Each evaluation instance is provided as one prompt containing all $N$ questions and their assigned scores. Specifically, question $i$ is formatted as:
\begin{quote}
\small
\texttt{Qi: [question text] (This question is worth [score] points)}
\end{quote}
The prompt instructs the model to maximize total score under a shared token budget, with optional strategy hints (planning, skipping expensive questions, and/or rechecking) depending on the experimental condition. The full prompt is shown in Figure~\ref{fig:inference_prompt}. More details on the optional strategy hints are included in Section~\ref{sec:test-taking-strategy}

\paragraph{Two-Phase Inference and Answer Forcing.}
Inference is performed in two phases. In Phase 1, the model generates free-form reasoning for the full exam prompt, with decoding capped at the global budget. In Phase 2, we ask the model for each question answer separately (\texttt{Q1}, \texttt{Q2}, \ldots, \texttt{QN}) using the Phase 1 reasoning as context. Each Phase 2 generation is constrained with guided decoding using regex\texttt{ \textbackslash boxed\{.\}}, and we extract the content inside \texttt{\textbackslash boxed\{\}} as the final answer. If Phase 1 stops due to budget, we append a model-specific end-thinking token before the per-question answer prompts to mimic that the reasoning process has completed, and explicitly tell the model its reasoning budget is used up.

\paragraph{Budget.}
For each evaluation instance, regardless of $N$, the model receives a total reasoning budget of 20{,}000 tokens in Phase 1. When this budget is exhausted, Phase 1 is truncated by the decoder's length limit; we then transition to Phase 2 and force per-question final answers as described above. Answers are saved as a JSON-serialized answer mapping keyed by question ID (\texttt{Q1}\ldots\texttt{QN}).
As Phase 2 incorporates regex-guided constrained decoding, every question receives an answer slot in the saved output whether the Phase 1 reasoning fully solved the question or not (i.e., no missing keys). 

% \paragraph{Saved Outputs and Missing-Answer Handling.}
% For each exam instance, we save the source file path, assigned scores, ground-truth answers, concatenated prompt text, full reasoning trace, and a JSON-serialized answer mapping keyed by question ID (\texttt{Q1}\ldots\texttt{QN}). Because Phase 2 always queries each question separately with forced answer format, every question receives an answer slot in the saved output (i.e., no missing keys).

\paragraph{Evaluation and Metrics.} The correctness of model responses on the evaluation instances is judged by LLM-as-a-judge using \texttt{GPT-5}~\citep{openai2025gpt5}. The detailed judge instruction is shown in Figure~\ref{fig:judge_prompt}. Performance is measured by score rate (\%), defined as 
\begin{equation}
    \text{Score Rate}=\frac{\text{Achieved score}}{\text{Max achievable score}}.
\end{equation}
For each question, the model receives full score if the answer is correct, and zero score otherwise. The max achievable score is the sum of the assigned scores for all questions within one evaluation instance. Since all compared conditions use the same global reasoning budget, score rate measures utility obtained under a fixed compute cost. The assigned scores represent task reward rather than token cost; reasoning cost is controlled separately by the budget. If budgets varied across methods, an additional utility-per-token metric would be necessary, but in our setting the fixed budget makes score rate directly comparable.




\subsection{Variables Affecting the Exam Design}
\label{sec:exam-design-choice}
% Our evaluation considers three key dimensions:

\paragraph{Score assignment strategies.}
To simulate exam conditions, each question is assigned a point value. We consider both difficulty-independent and difficulty-dependent scoring:
\begin{itemize}[leftmargin=10pt,itemsep=0pt,topsep=2pt]
    \item \textbf{Difficulty-independent scoring:} \textit{Random scoring}, where each question receives a value between 1 and 15, and \textit{fixed scoring}, where all questions are worth 10 points regardless of difficulty.
    \item \textbf{Difficulty-dependent scoring:} Scores are either \textit{proportional to difficulty} (harder questions yield more points) or \textit{inversely proportional to difficulty} (harder questions yield fewer points). The inverse setting tests whether the model avoids allocating large budget to low-reward difficult questions and instead prioritizes easier, higher-yield ones. 
\end{itemize}

In difficulty-proportional scoring, we map the sample's difficulty values to a 1--15 integer range in proportion to relative difficulty within the instance. Concretely, let $d_i$ be the original difficulty for question $i$ in the instance; we first linearly rescale all $d_i$ to the unit interval, i.e., normalizing per-sample difficulties to $[0,1]$. If all difficulties are identical in an instance, we fall back to a constant value (10 points per question). Otherwise, each score is computed as
\begin{equation}
    s_i = \left\lfloor 1 + 14\times \frac{d_i - d_{\min}}{d_{\max}-d_{\min}} \right\rfloor,
\end{equation}
where $d_{\min}$ and $d_{\max}$ are the (per-instance) minimum and maximum difficulties.

In difficulty-inverse scoring, easier questions receive larger point values while harder ones receive smaller values. Specifically, we compute \begin{equation}
    s_i = \left\lfloor 15 - 14\times \frac{d_i - d_{\min}}{d_{\max}-d_{\min}} \right\rfloor,
\end{equation}
again with the same per-instance normalization fallback to 10 points per question when all difficulties are equal.

\paragraph{Question ordering.}
Question order may influence allocation strategies, similar to its effect on human test-takers \cite{ANAYA2022102293, effect_of_q_order}. We evaluate three orderings:
\begin{itemize}[leftmargin=10pt,itemsep=0pt,topsep=2pt]
    \item \textbf{Increasing difficulty:} Easiest to hardest, mirroring typical exams.
    \item \textbf{Decreasing difficulty:} Hardest to easiest.
    \item \textbf{Random ordering:} Questions are shuffled independently of difficulty.
\end{itemize}
\subsection{Test-taking strategies.}
\label{sec:test-taking-strategy}
To examine how different test taking strategies affect the model's budget allocation behavior, we prompt the model with various instructions on how to smartly plan and spend its given budget. We compare implicit strategy as a baseline, where the model receives no explicit guidance on how to plan, prioritize, or skip questions, with explicit strategies that instruct the model to adopt common human test-taking techniques. These include asking the model to explicitly plan how to allocate its budget across questions, hinting the model to skip questions that appear too difficult or token-consuming, and instructing the model to double-check answers when there's ample budget. This setup allows us to evaluate whether providing strategic guidance improves the model’s ability to manage limited resources and maximize overall score.

We prompt the model with three different common human test-taking strategies as well as their combinations, namely:
\begin{itemize}[leftmargin=10pt,itemsep=0pt,topsep=2pt]
    \item \textbf{Explicit Planning}: The model is instructed to explicitly plan its spending of the given budget to maximize total score.
    \item \textbf{Skipping}: The model is hinted to skip questions that are too difficult or token-consuming.
    \item \textbf{Rechecking}: The model is instructed to check previous answers when there's ample budget.
\end{itemize}
The detailed prompts for each explicit strategy are included in Figure~\ref{fig:inference_prompt}.

\paragraph{Uniform-allocation baseline.}
To contextualize the model's implicit budget allocation behavior, we additionally evaluate a uniform-allocation baseline. Unlike the prompting strategies above, this baseline manually fixes the allocation policy: for each exam instance with $N$ questions and the same total budget of 20{,}000 tokens, we divide the budget evenly across questions and evaluate each question independently under its corresponding per-question budget. We then aggregate the earned points over all questions in the original exam instance, using the same assigned scores and score-rate metric as in the global-budget setting. This baseline represents a naive, difficulty-unaware allocation policy: it does not adapt to question difficulty, point value, or intermediate confidence, but it avoids spending a disproportionate amount of the shared budget on any single question.

% \subsection{Discriminative power test from Item-Response Theory}
% Additionally, we also plan to compute the IRT score for different evaluation settings in order to identify and compare the discriminative power among them. Specifically, we treat each exam paper (a list of questions) as an item and model as a test taker. 

\subsection{Results}
\label{sec:results}
We organize the results around the main factors in the exam-style evaluation. We first analyze how test-taking prompts, question ordering, exam length, model scale, and the uniform-allocation baseline interact under difficulty-proportional scoring. We then compare against fixed scoring to test whether the same allocation patterns persist when point values no longer signal question difficulty.

\subsubsection{The Effect of Test-taking Strategies, Question Ordering, and Exam Length}
Figure~\ref{fig:difficulty-proportional-results} reports the score rates achieved by the four evaluated models under difficulty-proportional scoring, across three exam lengths and three question orderings. Overall, human-like test-taking strategies provide modest but nontrivial gains in some settings, longer exams are consistently harder to solve under a shared reasoning budget, question ordering has a weak and model-dependent effect, and several global-budget prompting settings fail to outperform the naive uniform-allocation baseline.
\input{img_tab_tex/combined_difficulty_based}

\paragraph{Do human test-taking strategies improve overall performance?}
The effect of the test-taking strategy is present but not uniform across models and settings. The strongest gains generally come from the explicit-planning and rechecking conditions, especially for the two 14B models. These strategies appear to help the model distribute its budget more deliberately across questions, which is particularly useful when the exam is longer or when the question ordering front-loads difficult problems. By contrast, the skipping hint is less consistently beneficial: it can help in some cases by preventing wasted effort on low-yield questions, but it can also reduce performance when the model skips too aggressively. The baseline strategy remains competitive in several cases, indicating that the benefit of strategic prompting is real but limited rather than transformative.

\paragraph{Do models beat naive uniform allocation?}
The uniform-allocation baseline provides a simple lower bar for useful planning: a model that understands the global-budget setting should ideally allocate budget at least as effectively as an equal split across questions. Surprisingly, many global-budget settings underperform this baseline, especially for DeepSeek-R1-Distill-Qwen-7B and for longer exams with 10 or 20 questions. This suggests that current reasoning models do not reliably convert a global budget instruction into effective cross-question allocation. Instead, they may over-spend on early or difficult questions, leaving insufficient reasoning for the remaining exam. Since the uniform baseline is difficulty- and score-unaware, failing to beat it indicates that free-form global exam prompting can be actively less efficient than a naive fixed allocation policy. At the same time, the comparison should be interpreted as a budget-allocation diagnostic rather than a pure measure of mathematical ability, because the uniform baseline solves questions independently and therefore avoids cross-question distraction and truncation cascades.

\paragraph{What role does question ordering play?}
Question ordering has a weak and model-dependent effect in our setting. The figure does not show a consistent advantage for easy-to-hard, random, or hard-to-easy ordering across all models and exam lengths. In some cases, easy-to-hard appears slightly better, especially for the larger models, but the gaps are generally small compared with the effects of model scale and exam length. This suggests that, under a shared global token budget, the models are more sensitive to how much per-question budget is available than to the exact order in which questions appear.

\paragraph{The effect of exam length.}
Exam length has a strong negative effect on score rate. Across all three orderings, 5-question instances are easiest, 10-question instances are harder, and 20-question instances are the most challenging. This pattern is expected under a fixed global token budget: as the number of questions increases, the model must spread its reasoning more thinly across the exam. The longer exams therefore amplify the value of budget-aware behavior, but they also expose the limits of the model's ability to allocate effort perfectly. Even when the scoring scheme favors difficult questions, the normalized score rate tends to drop as the exam becomes longer.

\paragraph{Model comparisons.}
The 14B models achieve higher score rates than the 7B/8B models in nearly all conditions, showing that model capacity remains important under exam-style evaluation. Among the larger models, DeepSeek-R1-Distill-Qwen-14B usually attains the highest score rates, while Qwen3-14B remains competitive. The smaller models obtain lower absolute scores but show the same broad qualitative trends with respect to strategy, ordering, exam length, and the uniform-allocation baseline.

\subsubsection{The Effect of Score Assignment Strategies}
Figure~\ref{fig:fixed-score-results} reports the corresponding results under fixed score assignment, where every question is worth the same number of points. Compared with difficulty-proportional scoring, fixed scoring removes point value as an explicit allocation signal: a model no longer receives higher reward for solving harder questions, so a strong allocation policy should prioritize questions it can answer reliably and avoid spending excessive budget on any single difficult item. The main qualitative trends remain similar. Longer exams still substantially reduce score rate, larger models remain stronger, and question ordering continues to have no consistent global effect.
\input{img_tab_tex/combined_fixed}

\paragraph{Does fixed scoring change the role of uniform allocation?}
Under fixed scoring, the uniform-allocation baseline becomes an especially natural reference point because equal point values make equal budget division a plausible default strategy. The results again show that this simple policy is difficult for some global-budget prompting settings to beat, most clearly for DeepSeek-R1-Distill-Qwen-7B and in the 10- and 20-question regimes. This reinforces the conclusion from difficulty-proportional scoring: current models often fail to implement even a naive budget allocation policy when asked to solve the whole exam in one global reasoning trace. At the same time, stronger models and shorter exams more often exceed the uniform baseline, suggesting that global-budget prompting can be beneficial when the model has enough capacity and the budget pressure is moderate.

\paragraph{How does score assignment affect interpretation?}
The fixed-score setting complements difficulty-proportional scoring by isolating budget management from score-aware prioritization. In the difficulty-proportional setting, models can in principle use point values as a proxy for where higher payoff may lie; under fixed scoring, this incentive disappears, and the key challenge is avoiding inefficient over-allocation while maintaining broad coverage. The persistence of exam-length degradation and uniform-baseline underperformance across both scoring schemes suggests that the central failure mode is not only misunderstanding the score function, but also a more general weakness in cross-question budget control.

% In summary, the figure suggests that the exam design variables meaningfully shape performance, but the dominant effects are model scale and budget pressure. Strategy prompts help most when the model has enough capacity to exploit them, and question ordering matters most when the model must decide how to spend limited reasoning tokens early in the exam.




% Table~\ref{tab:baseline} presents the score rates achieved by the six evaluated models utilizing the baseline prompting strategy, delineated across three distinct question set sizes and three variations in question ordering. The score for each question is assigned proportional to the question difficulty.

% An analysis of these baseline results reveals several behavioral trends. Primarily, model performance exhibits a pronounced degradation as the question volume increases. Notably, all models demonstrate a substantial decline in score rates when scaling from 5 to 20 questions, confirming that effectively distributing a fixed budget across an expanding problem space constitutes a central challenge. This motivates us to investigate whether allocating a larger budget to instances with more questions can lead to improved performance. Furthermore, as one would expect, model scale significantly dictates efficacy: the two 14B parameter models consistently surpass their 7–8B counterparts by a substantial margin across all experimental configurations. Conversely, question ordering yields no consistent effect on performance outcomes. This suggests that, under the baseline prompting condition, the models fail to dynamically adjust their allocation strategies in response to varying progressions of problem difficulty. [We will test whether explicit guidance on how to plan and allocate the given budget would make the question ordering play a more consistent role in performance outcomes.]


==> archive_v1/sec/related.tex <==
\section{Related Work}

\subsection{Test-time Scaling \& Adaptive Reasoning}
Recent work has demonstrated that scaling inference-time computation can substantially improve the reasoning capabilities of large language models~\citep{snell2024scalingllmtesttimecompute,levi2024simplemodelinferencescaling,Guo_2025,muennighoff2025s1}. By allocating additional tokens at test time, models can engage in deliberative, chain-of-thought reasoning~\cite{wei2023chainofthoughtpromptingelicitsreasoning,kojima2023largelanguagemodelszeroshot,li2025schoenfeldsanatomymathematicalreasoning}, producing higher-quality solutions at the expense of increased computational cost. However, this paradigm introduces the risk of \emph{overthinking}~\cite{chen2025think23overthinkingo1like,fan2025missingpremiseexacerbatesoverthinking}, wherein models generate unnecessarily verbose reasoning traces even for straightforward problems, leading to excessive token consumption and inference cost.

A growing body of work~\citep{sui2025stopoverthinkingsurveyefficient, feng2025efficientreasoningmodelssurvey} seeks to improve efficiency and budget awareness of LLM reasoning. For example, L1~\citep{aggarwal2025l1controllinglongreasoning} introduces a reinforcement learning objective that jointly optimizes for accuracy and adherence to user-specified length constraints, ThinkPrune~\citep{hou2025thinkprunepruninglongchainofthought} continuously trains reasoning models with reinforcement learning under explicit token limits, and BudgetSteer~\citep{li2025steering} proposes a test-time guidance method that uses a lightweight predictor to model the remaining budget and steer the reasoning process toward a specified token budget without requiring additional training. Beyond fixed budgets, several approaches explore \emph{adaptive} allocation of reasoning effort via reinforcement learning~\citep{wang2025adareasoneradaptivereasoningenables, wu2025armadaptivereasoningmodel}. \citet{han2025tokenbudgetawarellmreasoning} proposes a framework that adaptively adjust the reasoning budget based on the difficulty estimation of the problem. However, these methods focus exclusively on allocating computation for individual questions in isolation. In contrast, our work addresses a more realistic setting in which models must dynamically and strategically distribute a shared, finite budget across \emph{multiple} questions, requiring global planning and strategic prioritization.

\subsection{Budget-constrained Evaluation}

Research in educational measurement and psychometrics~\cite{goldhammer2015measuring,vanderlinden2007hierarchical} has long established the importance of time-constrained assessment for evaluating human problem-solving ability. Yet the majority of existing LLM reasoning benchmarks, including GSM8k~\citep{cobbe2021trainingverifierssolvemath}, Omni-MATH~\cite{gao2024omnimathuniversalolympiadlevel}, and GPQA~\cite{rein2023gpqagraduatelevelgoogleproofqa}, evaluate solely on answer accuracy, imposing no constraint on the tokens a model may consume per question.
Recent efforts have begun to incorporate budget awareness into evaluation and training. \citet{ma2025reasoningmodelseffectivethinking} introduce a per-question token budget to compare thinking and non-thinking modes of reasoning models, while BudgetThinker~\citep{wen2025budgetthinkerempoweringbudgetawarellm} employs reinforcement learning to improve performance under fixed per-question budgets. At the multi-question level, the 2024 International Olympiad in Informatics imposed a shared global time constraint on all contestants, under which o1~\cite{openai2024o1} placed at the 49th percentile alongside human participants. Our work adopts a \emph{global} token budget across multiple questions as a more realistic evaluation setting, requiring models to strategically manage a finite shared resource.

% 1. While most benchmark don't
% 2. Efficient reasoning paper do have some per-question limit
% \cite{ma2025reasoningmodelseffectivethinking}
% 3. IOI limits the total amount of time. We argue that it is not a good option

% 4. Human do a time-constrained test and there are some benefits

==> archive_v1/sec/time.tex <==
\section{Timeline}

\begin{itemize}
    \item \textbf{Mar 6 - Mar 15: Proposal \& Baseline Setup.} Submit the initial proposal. Complete data preprocessing and establish the first-step deliverable by evaluating unconstrained baseline model performance.
    \item \textbf{Mar 16 - Mar 31: Core Experiments.} Evaluate difficulty-dependent scoring and question orderings (increasing, decreasing, random) under a fixed total budget.
    \item \textbf{Apr 1 - Apr 15: Strategy Evaluation \& Analysis.} Test explicit prompting strategies (e.g., planning and skipping). Finalize experiments and quantitatively analyze allocation behaviors.
    \item \textbf{Apr 16 - Apr 30: Report Drafting.} Draft the final project report, detailing the problem formulation, methodology, and empirical findings.
    \item \textbf{May 1 - May 11: Final Submission \& Poster Prep.} Submit the final report, design the poster, and prepare for the poster session.
\end{itemize}

==> img_tab_tex/baseline_orderings.tex <==
\begin{table*}[ht]
\centering

\footnotesize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}l*{9}{c}@{}}
\toprule
\textbf{Model}
  & \multicolumn{3}{c}{\textbf{5 Qs}}
  & \multicolumn{3}{c}{\textbf{10 Qs}}
  & \multicolumn{3}{c}{\textbf{20 Qs}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
 & \textbf{rand.} & \textbf{e$\rightarrow$h} & \textbf{h$\rightarrow$e}
 & \textbf{rand.} & \textbf{e$\rightarrow$h} & \textbf{h$\rightarrow$e}
 & \textbf{rand.} & \textbf{e$\rightarrow$h} & \textbf{h$\rightarrow$e} \\
\midrule
Qwen3-14B      & 25.9 & 24.6 & 21.4 & 17.2 & 15.3 & 13.6 &  7.6 & 11.6 & 10.8 \\
Qwen3-8B       & 13.7 & 12.8 & 17.9 &  8.8 &  8.6 &  7.6 &  7.5 &  7.0 &  5.2 \\
DS-R1-Llama-8B & 13.8 & 16.9 & 14.3 &  9.1 & 10.1 &  8.6 &  5.1 &  6.1 &  5.5 \\
DS-R1-Qwen-14B & 22.4 & 24.0 & 31.3 & 17.2 & 17.2 & 16.0 & 14.0 &  9.0 &  9.8 \\
DS-R1-Qwen-7B  & 10.6 & 13.1 & 15.6 &  7.7 &  5.6 &  3.3 &  3.1 &  3.0 &  2.1 \\
Llama-3.1-8B   &  7.8 &  5.5 &  3.9 &  7.2 &  5.5 &  2.8 &  3.3 &  4.3 &  3.3 \\
\bottomrule
\end{tabular}
\caption{Score rates (\%) under a fixed 10K token budget with no explicit guidance regarding budget allocation, shown separately for different question orderings. Within each question-count block, the 3 columns corresponds to random ordering (rand.), increasing difficulty (e$\rightarrow$h), and decreasing difficulty (h$\rightarrow$e). Overall, performance degrades as question count increases, larger models consistently outperform smaller ones, and question ordering has negligible impact, highlighting limitations in adaptive budget allocation.}
\label{tab:baseline}
\end{table*}


==> img_tab_tex/combined_difficulty_based.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/combined_grouped_stacked_plot_difficulty_based.pdf}
    \caption{Score rates under difficulty-proportional scoring. Rows show question ordering, model panels are separated by dashed lines, and bars compare strategy conditions across 5, 10, and 20-question exams. Red bars denote the uniform-allocation baseline, which splits the global budget evenly across questions and aggregates the resulting exam score. Overall, human-like test-taking strategies provide modest but nontrivial gains in some settings, longer exams are consistently harder to solve under a shared reasoning budget, but question ordering has a weak and model-dependent effect. Many model dynamic budget allocations fail to beat the uniform allocation baselines.}
    \label{fig:difficulty-proportional-results}
\end{figure*}


==> img_tab_tex/combined_fixed.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/combined_grouped_stacked_plot_fixed.pdf}
    \caption{Score rates under fixed scoring, where all questions receive equal point values. The red uniform-allocation baseline evenly splits the global budget across questions. This setting removes point-value variation, isolating budget management across equally rewarded questions. The same exam-length degradation and uniform-baseline underperformance persist even without score-based prioritization.}
    \label{fig:fixed-score-results}
\end{figure*}


==> img_tab_tex/explicit_plan_prompt.tex <==
\begin{figure}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\linewidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Prompt for Explicit Planning},
  fonttitle=\bfseries,
  % fontupper=\ttfamily
]
Each question has a different difficulty and may require a different amount of reasoning to answer correctly. You should plan your allocation/spending wisely to maximize the total score.


\end{tcolorbox}
\end{figure}

==> img_tab_tex/recheck_answer_prompt.tex <==
\begin{figure}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\linewidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Prompt for Rechecking Answers},
  fonttitle=\bfseries,
  % fontupper=\ttfamily
]
If you think you have more than enough budget, you may also recheck and refine your answers to early questions to further increase the chances of maximizing the total score, but keep in mind that the rechecking also consumes your output budget.


\end{tcolorbox}
\end{figure}

==> img_tab_tex/skip_question_prompt.tex <==
\begin{figure}[h]
\centering
\begin{tcolorbox}[
  enhanced,
  colframe=black!50,
  colback=white,
  coltitle=black,
  colbacktitle=black!20,
  width=\linewidth,
  arc=2mm,
  auto outer arc,
  boxrule=0.5pt,
  left=10pt,
  right=10pt,
  top=8pt,
  bottom=8pt,
  title=\textbf{Prompt for Question Skipping},
  fonttitle=\bfseries,
  % fontupper=\ttfamily
]
You may even choose to not answer some questions if you think the cost of answering them is too high compared to the potential score gain.


\end{tcolorbox}
\end{figure}

==> img_tab_tex/tab_crux_main.tex <==
\begin{table*}[t]
\centering
\small
\caption{\textbf{CRUXEval-O position and coverage} under \texttt{fixed}/\texttt{orig}/\texttt{baseline} with shared budget $B{=}3{,}000$. Token effort decreases with position while token-centroid solving order nearly follows the prompt exactly. Increasing $N$ sharply increases front-loading and zero-token questions. Asterisks denote $p<0.05$.}
\label{tab:crux-main}
\begin{tabular}{llrrrrrrr}
\toprule
\textbf{Model} & $\boldsymbol{N}$ & \textbf{Tok$\sim$Pos} & \textbf{Ord$\sim$Pos} & \textbf{F/B} & \textbf{Front} & \textbf{Zero} & \textbf{Hit $B$} & \textbf{Acc.} \\
\midrule
QW-14  & 10 & $-0.39^{*}$ & 1.00 & 1.76 & 63\% & 24\% & 88\% & 49.6\% \\
QW-14  & 20 & $-0.67^{*}$ & 1.00 & 5.22 & 83\% & 47\% & 98\% & 47.2\% \\
DQ-14  & 10 & $-0.16^{*}$ & 0.94 & 1.36 & 51\% & 23\% & 83\% & 39.8\% \\
DQ-14  & 20 & $-0.59^{*}$ & 1.00 & 3.89 & 76\% & 42\% & 100\% & 34.7\% \\
DSV4-F & 10 & $-0.20^{*}$ & 0.97 & 1.47 & 57\% & 19\% & 70\% & 86.2\% \\
DSV4-F & 20 & $-0.65^{*}$ & 1.00 & 4.07 & 79\% & 40\% & 100\% & 80.8\% \\
DSV4-P & 10 & $-0.13^{*}$ & 0.98 & 1.10 & 51\% & 8\% & 56\% & 92.8\% \\
DSV4-P & 20 & $-0.59^{*}$ & 1.00 & 2.68 & 71\% & 30\% & 96\% & 79.0\% \\
\bottomrule
\end{tabular}
\end{table*}


==> img_tab_tex/tab_crux_value_plan.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{\textbf{CRUXEval-O value-blindness and planning detail.} Panel (a) uses \texttt{random}/\texttt{orig}/\texttt{baseline}; points are independent of position. Panel (b) compares \texttt{fixed} allocation statistics at $N{=}20$ while reporting tokens$\sim$points from the matched \texttt{random} cell. Planning modestly flattens some models but does not induce value sensitivity.}
\label{tab:crux-value-plan}
\begin{minipage}[t]{0.34\textwidth}
\centering
\textbf{(a) Value correlations}\\[2pt]
\begin{tabular}{llrr}
\toprule
\textbf{Model} & $\boldsymbol{N}$ & \textbf{Tok$\sim$Pts} & \textbf{Ord$\sim$Pts} \\
\midrule
QW-14  & 10 & 0.05 & $-0.09$ \\
QW-14  & 20 & 0.03 & 0.01 \\
DQ-14  & 10 & $-0.06$ & $-0.03$ \\
DQ-14  & 20 & $-0.01$ & 0.05 \\
DSV4-F & 10 & $-0.06$ & $-0.02$ \\
DSV4-F & 20 & 0.01 & $-0.04$ \\
DSV4-P & 10 & $0.15^{*}$ & 0.10 \\
DSV4-P & 20 & 0.02 & $-0.04$ \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.64\textwidth}
\centering
\textbf{(b) Explicit planning at $N{=}20$}\\[2pt]
\begin{tabular}{llrrrrr}
\toprule
\textbf{Model} & \textbf{Strategy} & \textbf{Zero} & \textbf{Front} & \textbf{F/B} & \textbf{Tok$\sim$Pts} & \textbf{Acc.} \\
\midrule
QW-14  & baseline & 47\% & 83\% & 5.22 & 0.03 & 47.2\% \\
QW-14  & plan     & 44\% & 77\% & 4.31 & 0.00 & 46.7\% \\
DQ-14  & baseline & 42\% & 76\% & 3.89 & $-0.01$ & 34.7\% \\
DQ-14  & plan     & 40\% & 75\% & 3.72 & 0.07 & 36.6\% \\
DSV4-F & baseline & 40\% & 79\% & 4.07 & 0.01 & 80.8\% \\
DSV4-F & plan     & 42\% & 76\% & 4.19 & $-0.04$ & 78.5\% \\
DSV4-P & baseline & 30\% & 71\% & 2.68 & 0.02 & 79.0\% \\
DSV4-P & plan     & 30\% & 69\% & 2.48 & 0.01 & 83.0\% \\
\bottomrule
\end{tabular}
\end{minipage}
\end{table*}


==> img_tab_tex/tab_deconfound.tex <==
\begin{table}[t]
\centering
\small
\caption{Capability is not the bottleneck. Score rate (\%) under unlimited per-question inference (40{,}960 tok/q, isolated) vs.\ one shared 20k-token exam ($N{=}10$, \texttt{align}/\texttt{orig}, \texttt{baseline}). Same questions; the collapse under shared budget indicates allocation failure, not a math ceiling.}
\label{tab:deconfound}
\begin{tabularx}{\columnwidth}{@{}L R R@{}}
\toprule
Model & Unlimited per-Q & Shared budget \\
\midrule
DSV4-P & 89.4 & 47.5 \\
DSV4-F & 86.8 & 49.3 \\
QW-32 & 78.4 & 20.9 \\
QW-14 & 76.1 & 14.3 \\
QW-8  & 70.7 & 11.6 \\
DQ-14 & 60.1 & 27.5 \\
DQ-7  & 55.7 & 11.5 \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_density.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Value-density selection test at $N{=}10$ under the baseline prompt.
Among the $k$ questions in the work set, \texttt{ov\_dens} and \texttt{ov\_pos}
are the overlap with the top-$k$ questions by value density and by prompt
position; \texttt{chance} is $k/N$. \texttt{wf@0} and \texttt{wtok@0} are the
fraction of the work set and of reasoning tokens spent on density-zero items,
which the model answers incorrectly even unconstrained. Upper block:
\texttt{random}/\texttt{asc}, where point value is decoupled from position and
difficulty. Lower block: model means for the remaining scoring schemes.
Density never beats chance, while position always does.}
\label{tab:density}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Model & chance & ov\_dens & ov\_pos & wf@0 & wtok@0 \\
\midrule
DQ-7   & 0.62 & 0.62 & 0.86 & 0.39 & 0.51 \\
DQ-14  & 0.63 & 0.65 & 0.75 & 0.36 & 0.44 \\
QW-8   & 0.57 & 0.55 & 0.77 & 0.26 & 0.34 \\
QW-14  & 0.65 & 0.67 & 0.76 & 0.21 & 0.26 \\
QW-32  & 0.61 & 0.64 & 0.75 & 0.18 & 0.23 \\
DSV4-F & 0.55 & 0.53 & 0.76 & 0.17 & 0.26 \\
DSV4-P & 0.50 & 0.46 & 0.64 & 0.13 & 0.17 \\
\textbf{Mean} & \textbf{0.59} & \textbf{0.59} & \textbf{0.76} & \textbf{0.24} & \textbf{0.32} \\
\midrule
\multicolumn{6}{@{}l}{\emph{Mean over models, other scoring schemes}} \\
\texttt{fixed}   & 0.53 & 0.47 & 0.81 & 0.28 & 0.37 \\
\texttt{align}   & 0.51 & 0.46 & 0.78 & 0.29 & 0.37 \\
\texttt{reverse} & 0.54 & 0.53 & 0.75 & 0.27 & 0.35 \\
\bottomrule
\end{tabular}
\end{table}


==> img_tab_tex/tab_factor_summary.tex <==
\begin{table}[t]
\centering
\small
\caption{Experimental factors at a glance. Omni-MATH is the primary full-factorial domain ($B{=}20{,}000$). The CRUXEval-O generality check uses $N{\in}\{10,20\}$, $B{=}3{,}000$, \texttt{fixed}/\texttt{random}, \texttt{baseline}/\texttt{explicit\_plan}, and \texttt{orig} only.}
\label{tab:factor-summary}
\begin{tabularx}{\columnwidth}{@{}l L@{}}
\toprule
\textbf{Factor} & \textbf{Values / role} \\
\midrule
Exam length $N$ & Math: 5, 10, 20; CRUX: 10, 20 \\
Scoring & Math: \texttt{fixed}, \texttt{random}, \texttt{align}, \texttt{reverse}; CRUX: first two \\
Ordering & Math: \texttt{orig}, \texttt{asc}, \texttt{dsc}; CRUX: \texttt{orig} \\
Strategy & \texttt{baseline}, \texttt{explicit\_plan} (math skip/recheck/ALL in appendix) \\
Reference lines & unlimited per-Q (40{,}960 tok/q); uniform per-Q ($B/N$, isolated) \\
\midrule
Allocation metrics & token effort; front/back ratio; zero-token rate; solving-order $\rho$ \\
Consequence metrics & score rate; align$-$reverse tax; vs.\ uniform $\Delta$ \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_mechanism_summary.tex <==
\begin{table}[t]
\centering
\small
\caption{Two allocation behaviors $\times$ three signals. Mean Spearman $\rho$ over all six models and $N{\in}\{5,10,20\}$, \texttt{baseline}. Position/difficulty use partial $\rho$ under \texttt{fixed}/\texttt{orig}; value uses raw $\rho$ under \texttt{random}. Restricting to the four open-weight models shifts no cell by more than $0.04$.}
\label{tab:mechanism-summary}
\begin{tabularx}{\columnwidth}{@{}L cc cc@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{Token effort}} & \multicolumn{2}{c}{\textbf{Solving order}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{Signal} & $\rho$ & verdict & $\rho$ & verdict \\
\midrule
Position   & $-$0.38 & front-loads & $+$0.72 & prompt-seq. \\
Difficulty & $+$0.19 & reactive    & $+$0.09 & none \\
Value      & $+$0.04 & blind       & $-$0.07 & blind \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_n_scaling.tex <==
\begin{table}[t]
\centering
\small
\caption{Allocation failure worsens with $N$ (\texttt{fixed}/\texttt{orig}/\texttt{baseline}, open-model mean). Position dominance grows, difficulty sensitivity decays, coverage collapses.}
\label{tab:n-scaling}
\begin{tabularx}{\columnwidth}{@{}L R R R R@{}}
\toprule
$N$ & Pos$|$D & Diff$|$P & f/b & zero \\
\midrule
5  & $-$0.19 & $+$0.37 & 1.4$\times$ & 0.18 \\
10 & $-$0.38 & $+$0.20 & 2.5$\times$ & 0.35 \\
20 & $-$0.46 & $+$0.07 & 3.0$\times$ & 0.53 \\
\midrule
\multicolumn{5}{@{}l}{\footnotesize DSV4 at $N{=}20$: zero 0.60--0.69; f/b $\approx$15$\times$} \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_order_scoring.tex <==
\begin{table}[t]
\centering
\small
\caption{Order $\times$ scoring consequence (DSV4-F, \texttt{baseline}; score rate \%). \texttt{reverse}$\times$\texttt{asc} is the ``lucky'' cell: position-greedy solving meets easy=valuable scoring.}
\label{tab:order-scoring}
\begin{tabularx}{\columnwidth}{@{}L R R@{}}
\toprule
 & \texttt{align} & \texttt{reverse} \\
\midrule
\multicolumn{3}{@{}l}{\textit{$N{=}10$}} \\
\texttt{asc} & 47.4 & \textbf{77.9} \\
\texttt{dsc} & 44.3 & 55.9 \\
\midrule
\multicolumn{3}{@{}l}{\textit{$N{=}20$}} \\
\texttt{asc} & 32.9 & \textbf{64.2} \\
\texttt{dsc} & 36.4 & 48.4 \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_plan_intervention.tex <==
\begin{table}[t]
\centering
\small
\caption{Explicit planning flattens spend but does not strategize ($N{=}20$, \texttt{fixed}/\texttt{orig}, open-model mean vs.\ DSV4-F/P). Value $\rho$ stays $\approx 0$ under \texttt{random}.}
\label{tab:plan-intervention}
\begin{tabularx}{\columnwidth}{@{}L R R R R@{}}
\toprule
Condition & f/b & zero & ord$\rho$(pos) & val$\rho$ \\
\midrule
\multicolumn{5}{@{}l}{\textit{Open mean}} \\
baseline & 3.0$\times$ & 0.52 & 0.71 & $\approx 0$ \\
explicit\_plan & 1.7$\times$ & 0.29 & 0.63 & $\approx 0$ \\
\midrule
DSV4-F baseline & 14.9$\times$ & 0.69 & 0.92 & $\approx 0$ \\
DSV4-F plan & 5.2$\times$ & 0.51 & -- & $\approx 0$ \\
DSV4-P baseline & 15.1$\times$ & 0.60 & 0.66 & $\approx 0$ \\
DSV4-P plan & 12.5$\times$ & 0.60 & -- & $\approx 0$ \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_pos_diff.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Position dominates difficulty in token effort (\texttt{fixed}/\texttt{orig}/\texttt{baseline}). Partial Spearman $\rho$ (Pos$|$D, Diff$|$P), front/back token ratio (f/b), zero-token fraction, and solving-order $\rho$ vs.\ position and difficulty. $^{*}$ token partial $p{<}0.05$. Open-model mean plus representative rows; DSV4 rows at $N{=}20$. Full per-model grid in Appendix~\ref{append:correlations}.}
\label{tab:pos-diff}
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
Model & $N$ & Pos$|$D & Diff$|$P & f/b & zero & oPos & oDiff \\
\midrule
DQ-7  & 20 & $-$0.57$^{*}$ & $+$0.11$^{*}$ & 4.5 & 0.48 & 0.87 & $-$0.00 \\
QW-8  & 20 & $-$0.36$^{*}$ & $-$0.07$^{*}$ & 2.6 & 0.60 & 0.63 & 0.36 \\
\textit{Open mean} & -- & $-$0.34 & $+$0.21 & 2.2 & 0.29 & 0.70 & 0.11 \\
\midrule
DSV4-F & 20 & $-$0.59$^{*}$ & $+$0.03 & 14.9 & 0.69 & 0.92 & 0.17 \\
DSV4-P & 20 & $-$0.57$^{*}$ & $+$0.04 & 15.1 & 0.60 & 0.72 & 0.21 \\
\bottomrule
\end{tabular}
\end{table}


==> img_tab_tex/tab_solving_order.tex <==
\begin{table}[t]
\centering
\small
\caption{Solving-order stress test (\texttt{fixed}/\texttt{baseline}; token-centroid rank $\rho$ vs.\ prompt position). High $\rho$ under \texttt{dsc} (hard first) indicates position-lock, not strategic reordering.}
\label{tab:solving-order}
\begin{tabularx}{\columnwidth}{@{}L R R R@{}}
\toprule
Model & \texttt{asc} & \texttt{rand} & \texttt{dsc} \\
\midrule
DQ-7  & 0.82 & 0.86 & 0.85 \\
DQ-14 & 0.87 & 0.90 & 0.90 \\
QW-8  & 0.90 & 0.55 & 0.50 \\
QW-14 & 0.85 & 0.45 & 0.34 \\
\midrule
DSV4-F & 0.93 & 0.91 & 0.80 \\
DSV4-P & 0.82 & 0.65 & 0.79 \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_uniform.tex <==
\begin{table}[t]
\centering
\small
\caption{One-round shared budget vs.\ naive uniform per-Q ($B/N$, isolated), \texttt{align}/\texttt{orig}/\texttt{baseline}. Wins = models where the shared budget beats uniform; $\Delta$ = mean score-rate difference (shared $-$ uniform). This is not a universal upper bound---uniform also removes cross-question interference.}
\label{tab:uniform}
\begin{tabularx}{\columnwidth}{@{}c c c L@{}}
\toprule
$N$ & wins/7 & $\Delta$ (pts) & read \\
\midrule
5  & 4/7 & $+$2.6 & mixed; small-$N$ front-loading can help \\
10 & 3/7 & $-$0.4 & model-dependent \\
20 & 0/7 & $-$5.0 & shared budget net worse for all models \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_value_blind.tex <==
\begin{table}[t]
\centering
\small
\caption{Value-blindness under \texttt{random} scoring (points $\perp$ difficulty \& position). Mean Spearman $\rho$ of token effort and solving order vs.\ assigned points; \texttt{baseline}, mean over open models plus DSV4-F/P.}
\label{tab:value-blind}
\begin{tabularx}{\columnwidth}{@{}L R R@{}}
\toprule
$N$ & tok $\sim$ Pts & ord $\sim$ Pts \\
\midrule
5  & 0.02 & $-$0.03 \\
10 & 0.07 & $-$0.12 \\
20 & 0.11 & $-$0.11 \\
\midrule
DSV4 (all $N$) & $\approx 0$ (0/18 sig.) & $\approx 0$ \\
\bottomrule
\end{tabularx}
\end{table}


==> img_tab_tex/tab_value_tax.tex <==
\begin{table}[t]
\centering
\small
\caption{Align$\leftrightarrow$reverse as repricing, not reallocation. Score rate (\%) and value-blindness tax (align $-$ reverse), \texttt{baseline}/\texttt{orig}, mean over matched cells.}
\label{tab:value-tax}
\begin{tabularx}{\columnwidth}{@{}L R R R@{}}
\toprule
Model & align & reverse & tax \\
\midrule
QW-14 & 22.1 & 37.5 & $-$15.4 \\
DQ-14 & 25.4 & 39.1 & $-$13.7 \\
DSV4-F & 48.2 & 60.1 & $-$11.8 \\
QW-8  & 15.4 & 26.5 & $-$11.2 \\
DSV4-P & 48.4 & 57.5 & $-$9.1 \\
DQ-7  & 11.2 & 17.1 & $-$5.9 \\
\bottomrule
\end{tabularx}
\end{table}


==> sec/analysis.tex <==
\section{Analysis: Why Allocation Fails}
\label{sec:analysis}

We interpret the mechanism through a knapsack lens and separate control failures from metacognitive limits.

\subsection{Knapsack view and the greedy density heuristic}
The exam is a knapsack problem. The shared budget $B$ is the capacity, a question's stated point value $s_i$ is its value, and the number of tokens the model would need to solve it is its weight $w_i$. Allocating strategically means selecting a subset of questions whose combined cost fits within the budget and whose combined value is as large as possible. The classic greedy heuristic for this problem takes questions in decreasing order of value density $s_i/w_i$. Our central finding, restated in these terms, is that models fail even this heuristic: they select by prompt position rather than by density.

Testing this requires an estimate of $w_i$, which the exam runs themselves cannot provide, since a question that receives no tokens reveals nothing about what it would have cost. We therefore introduce an \emph{unconstrained} reference condition, in which each question is presented on its own with an allowance of 40{,}960 tokens and no mention of any budget. This condition plays two roles. It supplies the per-question token count we use as a cost estimate, and it identifies the questions the model cannot answer even without competition; those are assigned zero density, because no amount of budget buys their points.

Table~\ref{tab:density} reports the resulting test. Among the questions a model actually works on, overlap with the top-$k$ items by density averages 0.60, essentially the chance level of 0.59 implied by the size of the work set. Overlap with the top-$k$ by prompt position is 0.76, well above chance. Models also commit substantial effort to items of zero density: 22\% of the work set, and 30\% of all reasoning tokens, go to questions that remain wrong even in the unconstrained condition.

\input{img_tab_tex/tab_density}

\subsection{Two failure types: ignoring given values vs.\ estimating latent costs}
Point values $s_i$ are \textbf{in the prompt}---value-blindness is a control/attention failure. Costs $w_i$ (tokens needed to solve) are \textbf{latent}---strategic allocation requires metacognitive self-estimation of per-question solvability.

\subsection{Cost endogeneity}
The unconstrained condition is a calibration device, not an oracle. Its token counts are inflated by overthinking, and what a model spends when nothing competes for the budget is not what the same question would require under pressure. These counts therefore should not be read as true knapsack weights, and we do not use them to compute an optimal allocation under $B$ or to report how far a model falls short of one. What they support is ordinal: whether the observed selection tracks density at all, and which items are unsolvable regardless of spending. The conclusions that rest on this---value-blindness, position-greed, the worsening with $N$, and the flattening effect of planning---do not depend on the absolute cost scale. Recovering genuine weights would require estimating each question's solve probability $P_i(t)$ at several budgets.

\subsection{Reactive sensing vs.\ prospective estimation}
The positive tokens$\sim$difficulty correlation is \emph{reactive} sunk-cost sensing (more tokens as a question proves hard), not prospective estimation of which items to attempt. Under budget, reactive sensing can be harmful: the harder it feels, the more the model pours in---often into low-density items. This also explains inconsistent gains from skip hints: skipping requires prospective cost estimates the model lacks.

\subsection{Future probes}
Brief future directions: (i) prospective per-question difficulty/token estimates before solving; (ii) plan-vs-execution adherence under \texttt{explicit\_plan}. We do not present these as current results.


==> sec/exp.tex <==
\section{Experiments}
 
\paragraph{Benchmark and models.}
 
We construct exam-style evaluation sets by randomly sampling and concatenating problems from Omni-MATH~\citep{gao2024omnimathuniversalolympiadlevel}, an olympiad-level mathematical reasoning benchmark. Each evaluation instance consists of a set of $N$ questions bundled into a single prompt, where $N \in \{5, 10, 20\}$. This range is chosen to simulate exams of varying length and to test how models cope with increasing numbers of competing questions under a shared budget. Each question is assigned a point value and a difficulty label drawn from the original benchmark metadata.
 
We evaluate six open-weight language models spanning two parameter scales: four 7--8B models (Llama-3.1-8B-Instruct~\citep{grattafiori2024llama}, DeepSeek-R1-Distill-Qwen-7B, DeepSeek-R1-Distill-Llama-8B~\citep{guo2025deepseek}, and Qwen3-8B~\citep{yang2025qwen3}) and two 14B models (DeepSeek-R1-Distill-Qwen-14B~\citep{guo2025deepseek} and Qwen3-14B~\citep{yang2025qwen3}).
 
All models are served locally using vLLM~\citep{kwon2025vllm} with a fixed output token budget of 10{,}000 tokens.
 
\paragraph{Question Ordering}
 
To investigate whether the presentation order of questions affects a model's allocation strategy, we evaluate each model under three orderings:
\begin{itemize}
    \item \textbf{As-is (\texttt{asis})}: The original order from the sampled question set.
    \item \textbf{Ascending difficulty (\texttt{difficulty\_asc})}: Questions sorted from easiest to hardest.
    \item \textbf{Descending difficulty (\texttt{difficulty\_desc})}: Questions sorted from hardest to easiest.
\end{itemize}
 
\paragraph{Prompting Strategy (Baseline)}
 
In the baseline setting (\texttt{one\_round\_baseline}), the model receives a single prompt containing all $N$ questions along with an instruction specifying the total token budget. No additional guidance is provided regarding how to plan, prioritize, or skip questions. This serves as the control condition against which more elaborate prompting strategies are compared.
 
\paragraph{Evaluation}
 
Model outputs are evaluated using GPT as a judge model. For each question, the judge compares the model's answer against the reference solution and assigns a binary correctness label. We report two metrics:
\begin{itemize}
    \item \textbf{Accuracy (score rate)}: The fraction of total available points earned by correctly answered questions.
    \item \textbf{Budget compliance}: The fraction of evaluation instances in which the model's output stays within the 10{,}000-token budget.
\end{itemize}
 
% ============================================================
 
\subsection{Results}
\label{sec:baseline}
 
Table~\ref{tab:baseline} summarizes the accuracy of all six models under the baseline prompting strategy across three question set sizes and three question orderings.

 
 
Several trends emerge from the baseline results. Accuracy degrades sharply as the number of questions grows, with all models showing a substantial drop from 5 to 20 questions, confirming that distributing a fixed budget across more problems is the central challenge. The two 14B models consistently outperform all 7--8B models by a clear margin across every setting. Budget compliance is nearly zero for all models except Llama-3.1-8B-Instruct, which achieves 24--45\% compliance but at the cost of the lowest accuracy, suggesting a trade-off between respecting the budget and producing substantive reasoning. Question ordering (\texttt{asis}, \texttt{difficulty\_asc}, \texttt{difficulty\_desc}) has no consistent effect on performance, indicating that models do not adapt their allocation strategy to the difficulty progression under the baseline prompt.




==> sec/method.tex <==
% DEPRECATED (2026-07-10): split into sec/setup.tex + sec/results.tex.
% Prior version archived in paper/archive_v1/sec/method.tex


==> sec/results.tex <==
\section{Can LRMs Ration Test Time Compute Across Questions?}
\label{sec:results}

Under a shared budget, reasoning models behave like greedy sequential solvers. We build the diagnosis in six steps: the collapse is not a math ceiling (\S\ref{sec:results-deconfound}); allocation is driven by position rather than value or difficulty (\S\ref{sec:results-mechanism}); the failure worsens with the number of competing questions (\S\ref{sec:results-scaling}); prompting the model to plan flattens spend without making it strategic (\S\ref{sec:results-plan}); downstream score effects follow from this fixed policy (\S\ref{sec:results-consequences}); and a code-reasoning check tests whether the mechanism extends beyond math (\S\ref{sec:results-crux}). Throughout, the API frontier models DSV4-F/P track the open-model pattern: higher single-question capability does not buy strategic multi-question rationing.

\subsection{Capability is not the bottleneck}
\label{sec:results-deconfound}

\begin{finding}
\findinglabel Shared-budget collapse is not an inability to solve the items. Models that answer 56--89\% of questions correctly in isolation earn only 12--49\% of the points when the same questions share one budget.
\end{finding}

Table~\ref{tab:deconfound} contrasts unlimited per-question inference with a single shared-budget exam at $N{=}10$ (\texttt{align}/\texttt{orig}, \texttt{baseline}). Open models solve 56--78\% of items with unlimited per-question budget but earn only 12--28\% under the shared budget; DSV4-F/P reach 87--89\% in isolation yet fall to $\approx$48--49\% shared---the same qualitative collapse at far higher capability. The remaining sections therefore diagnose \emph{allocation}, not competence.

\input{img_tab_tex/tab_deconfound}

\subsection{What drives allocation? Two behaviors, three signals}
\label{sec:results-mechanism}

\begin{finding}
\findinglabel Both \emph{how much} budget a question receives and \emph{when} it is worked on are governed by prompt position, not by point value or difficulty. Difficulty enters token effort only weakly and reactively; value is ignored entirely.
\end{finding}

\subsubsection{Unified summary}
We separate allocation into two behaviors---token effort (how much budget a question receives) and solving order (when it is worked on)---and test each against three candidate signals: prompt position, difficulty, and assigned points. Table~\ref{tab:mechanism-summary} summarizes the mean correlations over all six models. Both behaviors track position and ignore value; difficulty leaks into token effort only reactively. Restricting the means to the open-weight models leaves the pattern unchanged, with slightly weaker position dominance.

\input{img_tab_tex/tab_mechanism_summary}

\subsubsection{Position and difficulty}
Under \texttt{fixed}/\texttt{orig}, difficulty is decoupled from prompt position, so partial Spearman $\rho$ cleanly separates the two. Token effort shows a growing negative Pos$|$D correlation (front-loading) and a small positive Diff$|$P that decays with $N$ (Table~\ref{tab:pos-diff}; full grids in Appendix~\ref{append:correlations}). Solving-order $\rho$ against position averages 0.70 for open models and 0.79 for DSV4. At $N{=}20$, DSV4 front/back token ratios reach $\approx$15$\times$ with 60--69\% zero-token questions---more extreme than open models despite higher capability.

\input{img_tab_tex/tab_pos_diff}

\subsubsection{Value-blindness}
Under \texttt{random} scoring, points are assigned independently of both difficulty and position, giving the cleanest test of value-awareness. Token effort and solving order correlate with points at $\rho{\approx}0$ across all $N$ and strategies; for DSV4, 0 of 18 cells are significant (Table~\ref{tab:value-blind}). A positive tokens$\sim$difficulty correlation is \emph{not} value-awareness---harder items consume more tokens regardless of their point value.

\input{img_tab_tex/tab_value_blind}

\subsubsection{Solving-order stress test}
Presenting the hardest questions first (\texttt{dsc}) is the adversarial test for order. DeepSeek models remain position-locked ($\rho{\approx}0.86$--0.91), grinding through hard items in order; Qwen partially reorders ($\rho{\approx}0.29$--0.46 at $N{=}20$) but gains no score (Table~\ref{tab:solving-order}). Reordering, where it occurs, is reactive deferral of hard front items, not strategic prioritization by value or density.

\input{img_tab_tex/tab_solving_order}

\noindent\textit{Synthesis: position substitutes for value and difficulty in both behaviors.}

\subsection{The failure worsens with the number of competing questions}
\label{sec:results-scaling}

\begin{finding}
\findinglabel The pathology intensifies exactly where allocation matters most: as $N$ grows, position dominance strengthens, difficulty sensitivity decays toward zero, and over half the exam receives no reasoning at all.
\end{finding}

Table~\ref{tab:n-scaling} tracks open-model means as $N$ increases from 5 to 20: Pos$|$D strengthens ($-$0.19 $\to$ $-$0.46), Diff$|$P decays ($+$0.37 $\to$ $+$0.07), the front/back ratio rises (1.4$\times$ $\to$ 3.0$\times$), and the zero-token fraction reaches 0.53. DSV4 is worse still on coverage at $N{=}20$ (0.60--0.69 zero-token). More capable models do not escape the pathology---frontier models can look \emph{worse} on coverage precisely because they front-load more aggressively.

\input{img_tab_tex/tab_n_scaling}

\subsection{Prompting to plan does not induce strategic allocation}
\label{sec:results-plan}

\begin{finding}
\findinglabel Explicitly instructing the model to plan its budget makes spending more \emph{uniform} (less front-loading, better coverage) but no more \emph{strategic}: value and difficulty sensitivity are unchanged.
\end{finding}

Comparing \texttt{baseline} with \texttt{explicit\_plan} at $N{=}20$ (Table~\ref{tab:plan-intervention}), open models cut the front/back ratio from 3.0$\times$ to 1.7$\times$ and the zero-token rate from 0.52 to 0.29, yet value $\rho$ stays $\approx 0$. DSV4-F responds partially (zero 0.69$\to$0.51; f/b 14.9$\times$$\to$5.2$\times$), while DSV4-P barely moves. The resulting \emph{near-uniform} spending is a consequence of the plan prompt specifically, not a property of default behavior.

\input{img_tab_tex/tab_plan_intervention}

\subsection{Score consequences of a position-greedy policy}
\label{sec:results-consequences}

\begin{finding}
\findinglabel Downstream score effects under alternate scorings and orderings are \emph{repricings} of a fixed solved set, not evidence of value-aware reallocation. The comparison to a uniform baseline is $N$-dependent, not a universal ceiling.
\end{finding}

\subsubsection{Align $\leftrightarrow$ reverse as repricing}
The value-blindness \emph{tax} (align score $-$ reverse score, on matched cells) is negative for every model (Table~\ref{tab:value-tax}): \texttt{reverse} scores higher because models keep solving the same easy questions---cheap under \texttt{align}, valuable under \texttt{reverse}---without reorganizing. Correct-set overlap across the two scorings is high ($\approx$0.86 at $N{=}10$) while work-set overlap is lower ($\approx$0.68); effort flips track point flips only weakly ($\rho{\approx}0.2$, 55\% directional). Instability across runs is not value-responsiveness.

\input{img_tab_tex/tab_value_tax}

\subsubsection{Order $\times$ scoring}
Table~\ref{tab:order-scoring} reports DSV4-F score rates under \texttt{baseline}. The \texttt{reverse}$\times$\texttt{asc} cell (easy questions first, easy questions worth most) is the highest at every $N$, $+$15--30 points over \texttt{align}$\times$\texttt{asc}: position-greedy solving happens to meet favorable scoring. The mirror-image \texttt{reverse}$\times$\texttt{dsc} cell is adversarial, forcing the model to grind worthless hard front items.

\input{img_tab_tex/tab_order_scoring}

\subsubsection{Uniform baseline is an $N$-dependent reference}
One-round shared budget versus naive uniform per-Q ($B/N$, isolated prompts) is mixed at small $N$ (4/7 wins at $N{=}5$, mean $+$2.6 pts) but uniformly worse at $N{=}20$ (0/7 wins, mean $-$5.0; Table~\ref{tab:uniform}). DSV4 loses to uniform at every $N$. We do \emph{not} claim a universal ``loses to uniform'': the uniform baseline also removes cross-question interference, so it is not a clean allocation oracle. Our mechanism claims (\S\ref{sec:results-mechanism}--\ref{sec:results-plan}) do not depend on beating it. Demoted score-rate bar charts appear in Appendix~\ref{append:score-rates}.

\input{img_tab_tex/tab_uniform}

\subsubsection{Ordering and strategy prompts on score}
Effects of ordering and of skip/recheck hints on the final score are weak and inconsistent, because the underlying allocation policy barely changes (the one exception being \texttt{explicit\_plan}'s flattening). We therefore refer back to \S\ref{sec:results-mechanism}--\ref{sec:results-plan} rather than re-analyzing every score bar.

\subsection{Cross-domain check: CRUXEval-O}
\label{sec:results-crux}

\begin{finding}
\findinglabel The same allocation pathology appears in code output prediction under a pressure-matched shared budget: effort is position-greedy, point values are ignored, coverage worsens with $N$, and planning flattens rather than strategizes.
\end{finding}

CRUXEval-O provides a deliberately narrower external-validity check rather than a co-equal second domain. Averaged over four models and $N{\in}\{10,20\}$ under \texttt{baseline}, token effort correlates with prompt position at $\rho{=}-0.42$ and solving order at $\rho{=}0.98$ (Table~\ref{tab:crux-main}). Under \texttt{random} scoring, the corresponding value correlations are only $0.02$ for effort and $-0.01$ for order. Thus near-perfect prompt-sequential solving coexists with no systematic response to stated points. One weak exception---DSV4-P effort at $N{=}10$, $\rho{=}0.15$---does not recur at $N{=}20$ or in solving order.

\input{img_tab_tex/tab_crux_main}

The capability de-confound also transfers. At $N{=}10$, QW-14 falls from 88.6\% unlimited per-Q accuracy to 49.6\% under the shared budget; DQ-14 falls from 81.0\% to 39.8\%. As competition doubles, zero-token questions rise from 8--24\% at $N{=}10$ to 30--47\% at $N{=}20$, front-half token share rises from 51--63\% to 71--83\%, and 96--100\% of runs hit the shared budget. These magnitudes differ from math, but the direction of every mechanism signal agrees.

Planning again changes spread, not priorities. At $N{=}20$, \texttt{explicit\_plan} modestly reduces front-loading for QW-14 (front/back 5.22$\to$4.31), DQ-14 (3.89$\to$3.72), and DSV4-P (2.68$\to$2.48), while DSV4-F remains essentially unchanged (4.07$\to$4.19). Across all four models, tokens$\sim$points stays near zero ($-0.04$ to $0.07$) and accuracy changes inconsistently. Under a pressure-matched budget, CRUXEval-O therefore reproduces the position-greedy, value-blind, $N$-worsening, plan-flattens pattern---including on frontier DSV4---showing that the allocation failure is not a math artifact.


==> sec/results_new.tex <==
\section{Can Reasoning Models Ration Shared Compute?}
\label{sec:results}

Our analysis proceeds through four questions. We first examine where models spend their tokens and what signals govern that allocation. We then ask how the behavior changes as more questions compete for the same budget, whether explicit planning improves the allocation policy, and how the resulting behavior affects the final score. A cross-domain check on code reasoning closes the section.

Some patterns are consistent across these analyses: models approach the exam largely as a sequence of independent questions. They devote substantial effort to questions near the beginning of the prompt, often leave later questions untouched, and respond only weakly to either difficulty or point value.

\subsection{RQ1: What Governs the Allocation of Reasoning?}
\label{sec:allocation_results}

To examine how the shared budget is distributed across questions, we study two complementary aspects of allocation:

\begin{itemize}[leftmargin=12pt,itemsep=-2pt,topsep=1pt]
    \item \textbf{Token effort:} how much reasoning a question receives;
    \item \textbf{Solving order:} when the model substantively works on it.
\end{itemize}

Both are computed from the marker segmentation of Section~\ref{sec:allocation}. Let $S_i$ be the set of reasoning segments attributed to question $i$, where each segment $s$ is a sequence of tokens of length $\tau_s$ that begins at position $p_s$. The token effort $t_i$ on question $i$ is the total attributed length across different reasoning segments of the question,
\begin{equation}
    t_i = \sum_{s\in S_i}\tau_s ,
    \label{eq:token_effort}
\end{equation}
and the \emph{zero-token rate} is the fraction of questions with $t_i=0$. Since a question can be mentioned in the plan but never allocated real resolving effort, we also define the \emph{work set}
\begin{equation}
    W = \bigl\{\, i \;|\; t_i \ge 200 \ \text{ or } \ |S_i| \ge 2 \,\bigr\},
    \label{eq:work_set}
\end{equation}
which separates substantive attempts from brief references and provides a stricter measure of coverage than the zero-token rate.

Solving order is then defined on the work set. We locate question $i$ by the token-weighted centroid of its segments,
\begin{equation}
    c_i = \frac{\sum_{s\in S_i}\tau_s\,p_s}{\sum_{s\in S_i}\tau_s} ,
    \label{eq:centroid}
\end{equation}
and rank the questions in $W$ by ascending $c_i$. The resulting rank is the solving order. Centroids keep an early mention from displacing a question that is mostly worked on later, and restricting to $W$ keeps a question that is merely enumerated in an opening pass from being ranked ahead of questions that actually received effort.

Finally, we summarize front-loading through the ratio
\begin{equation}
    R_{\mathrm{FB}}
    =
    \frac{
        \frac{1}{\lfloor N/2\rfloor}
        \sum_{i=1}^{\lfloor N/2\rfloor}t_i
    }{
        \frac{1}{N-\lfloor N/2\rfloor}
        \sum_{i=\lfloor N/2\rfloor+1}^{N}t_i
    }.
    \label{eq:front_back}
\end{equation}
A value above one means that questions in the first half of the prompt receive more tokens on average than those in the second half.

We ask whether these behaviors are governed by three possible signals: presentation position, question difficulty, and point value. Figure~\ref{fig:allocation_correlations} reports these correlations for every model and exam length, together with marginal means over models, over exam lengths, and over both. Token effort decreases with prompt position, while solving order closely follows it. Difficulty has a weaker relationship with effort and almost no relationship with solving order. Point value is essentially ignored by both.

\subsubsection{Position Dominates Difficulty}
\label{sec:position_difficulty}

To separate prompt position from difficulty, we use fixed scoring and random question order. In this condition, all questions have the same value and their positions are independent of their difficulty. We then compute partial Spearman correlations between token effort and position while controlling for difficulty, and between token effort and difficulty while controlling for position.

Figure~\ref{fig:allocation_correlations} shows that position is the stronger signal across models and exam lengths. Averaged over the open models and all exam lengths, the partial correlation between token effort and position is $-0.33$, against $+0.18$ for difficulty: later questions systematically receive fewer tokens. The per-length means over all seven models make the scaling especially clear: as $N$ grows from 5 to 20, the effort--position correlation strengthens from $-0.25$ to $-0.47$, while the effort--difficulty correlation falls from $+0.30$ to $+0.04$.

This positive difficulty effect should not be interpreted as strategic prioritization. It is more consistent with a reactive process: once the model begins a difficult question, it tends to spend longer on it. Difficulty does not strongly determine which questions are attempted first. Across the same models and exam lengths, the mean correlation between solving order and difficulty is only $0.09$, whereas solving order and prompt position correlate at $0.68$.

The API models show the same behavior more strongly. At $N=20$, DSV4-F and DSV4-P spend roughly 16 times as many tokens on the first half of the prompt as on the second. Between 61\% and 69\% of questions receive no attributed reasoning at all. Their greater single-question capability therefore does not translate into broader or more selective coverage; instead, they front-load particularly aggressively.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/allocation_corr_heatmap.pdf}
    \caption{
        Allocation correlations by model and exam length under the
        baseline prompt. Each panel relates token effort and solving
        order to position, difficulty, and point value. For position
        and difficulty, effort cells are partial Spearman correlations
        under fixed scoring and random question order; order cells are
        mean per-exam Spearman correlations in the same condition.
        Point-value cells use raw correlations under random scoring,
        where points are independent of position and difficulty.
        Solving order ranks the work set of Eq.~\ref{eq:work_set} by
        token-weighted centroid. The rightmost column averages the seven
        models at each $N$, the bottom row averages the three exam
        lengths for each model, and the bottom-right panel averages
        every model and exam length.
        Blue denotes negative and red positive correlation.
    }
    \label{fig:allocation_correlations}
\end{figure*}

The solving-order results make the sequential tendency especially clear. The consistently red position--order cells show that, even under random order, models largely work through questions in the order in which they appear. This remains true even though the prompt never instructs the model to follow that order.

\subsubsection{Models Do Not Respond to Point Value}
\label{sec:value_blindness}

Position-greedy behavior is not necessarily irrational if early questions happen to be more valuable. We therefore turn to random scoring, where each question's point value is assigned independently of both difficulty and position. This condition provides the cleanest test of whether the model uses the values explicitly stated in the prompt.

As shown by the pale point-value row in Figure~\ref{fig:allocation_correlations}, the answer is largely no. Averaged over all seven models, the effort--point correlation ranges only from $0.02$ to $0.09$ across exam lengths, while the order--point correlation ranges from $-0.09$ to $-0.03$. These effects are far weaker than the position correlations. The API models follow the same pattern: all six baseline cells shown in the figure are close to zero, and across their broader 18 model-by-length-by-strategy cells, none exhibits a statistically significant relationship between point value and token effort.

A model can therefore spend more tokens on difficult questions without being value-aware. Difficulty is experienced while solving; point value is given in advance. The former can increase effort reactively, while the latter would require the model to use the scoring objective to decide where effort should go. We observe little evidence of that second behavior.

\subsubsection{Hard-First Ordering Provides a Stress Test}
\label{sec:ordering_stress}

The decreasing-difficulty condition places the hardest questions at the beginning of the prompt. This creates an adversarial ordering for a sequential solver: following the prompt means consuming a large fraction of the budget before reaching easier questions.

Table~\ref{tab:order_stress} reports the correlation between prompt position and token-centroid solving order. DeepSeek-R1-Distill models remain almost completely position-locked across all orderings, including when the hardest questions come first. The API models also remain strongly sequential.

Qwen models depart more from prompt order in the hard-first condition, particularly at $N=20$. However, this reordering does not yield corresponding score improvements. The behavior appears to reflect local deferral after a difficult question has already been encountered, rather than prospective prioritization based on expected value or cost.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{7pt}
    \begin{tabular}{lrrr}
        \toprule
        \textbf{Model}
        & \textbf{Easy first}
        & \textbf{Random}
        & \textbf{Hard first} \\
        \midrule
        DQ-7   & 0.82 & 0.86 & 0.85 \\
        DQ-14  & 0.87 & 0.90 & 0.90 \\
        QW-8   & 0.90 & 0.55 & 0.50 \\
        QW-14  & 0.85 & 0.45 & 0.34 \\
        QW-32  & 0.80 & 0.40 & 0.26 \\
        DSV4-F & 0.93 & 0.91 & 0.80 \\
        DSV4-P & 0.82 & 0.65 & 0.79 \\
        \bottomrule
    \end{tabular}
    \caption{
        Spearman correlation between prompt position and
        token-centroid solving order under fixed scoring and the
        baseline prompt. Higher values indicate that the model follows
        the presented order more closely.
    }
    \label{tab:order_stress}
\end{table}

Taken together, these results identify presentation position as the dominant organizing signal. Difficulty affects how long a model continues once it has started, but has much less influence on when the question is attempted. Point value has almost no detectable effect on either decision.

\subsection{RQ2: Does the Failure Worsen as More Questions Compete?}
\label{sec:scaling_n}

The need for allocation becomes more important as the exam grows. With only a few questions, even a simple sequential strategy may reach most of the paper. With many questions, early overspending can prevent the model from considering a substantial fraction of the available opportunities.

Table~\ref{tab:n_scaling} shows exactly this progression for the open models. As $N$ increases from 5 to 20, the partial correlation between token effort and position strengthens from $-0.21$ to $-0.42$. At the same time, the relationship between effort and difficulty weakens from $+0.33$ to $+0.04$. The front/back ratio more than doubles, and the mean zero-token rate reaches 51\%.

Thus, increasing the number of questions does not merely spread a fixed budget more thinly. It changes the allocation pattern itself. Models become more dependent on position and less responsive to question-specific characteristics precisely when selective allocation would be most valuable.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{crrrr}
        \toprule
        $\boldsymbol{N}$
        & \textbf{Pos.\,$|$\,Diff.}
        & \textbf{Diff.\,$|$\,Pos.}
        & $\boldsymbol{R_{\mathrm{FB}}}$
        & \textbf{Zero} \\
        \midrule
        5  & $-0.21$ & $+0.33$ & $1.4\times$ & 0.16 \\
        10 & $-0.35$ & $+0.17$ & $2.3\times$ & 0.33 \\
        20 & $-0.42$ & $+0.04$ & $3.1\times$ & 0.51 \\
        \bottomrule
    \end{tabular}
    \caption{
        Open-model means under fixed scoring, random order, and
        the baseline prompt. Position dominance increases with exam
        length, while difficulty sensitivity and coverage decline.
        At $N=20$, DSV4-F/P have zero-token rates of 0.69 and 0.61
        and front/back ratios of approximately $16\times$.
    }
    \label{tab:n_scaling}
\end{table}

The API models reinforce this conclusion. At $N=20$, they leave 60\%--69\% of questions without attributed reasoning and allocate approximately 15 times more effort to the front half than to the back half. Stronger single-question reasoning does not remove the allocation failure; in this case, it accompanies even more concentrated spending.

\subsection{RQ3: Does Explicit Planning Improve Allocation?}
\label{sec:planning}

The baseline prompt tells the model about the shared budget and the goal of maximizing total score, but it does not explicitly ask for a budget plan. We therefore test whether a direct instruction to plan allocation before solving can change the resulting behavior.

The intervention does have an effect, but a limited one. As Table~\ref{tab:planning} shows, explicit planning makes spending more even. For the open-weight models at $N=20$, the mean front/back ratio falls from $3.0\times$ to $1.7\times$, while the zero-token rate decreases from 0.52 to 0.29. The solving order also becomes somewhat less tied to prompt position.

DSV4-F responds in the same direction, though less strongly: its front/back ratio falls from $14.9\times$ to $5.2\times$, and its zero-token rate falls from 0.69 to 0.51. DSV4-P changes little.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{llrrrc}
        \toprule
        \textbf{Model}
        & \textbf{Prompt}
        & $\boldsymbol{R_{\mathrm{FB}}}$
        & \textbf{Zero}
        & $\boldsymbol{\rho(\text{order},\text{pos.})}$
        & $\boldsymbol{\rho(\text{effort},\text{points})}$ \\
        \midrule
        Open mean
        & Baseline
        & $3.1\times$ & 0.51 & 0.64 & $\approx 0$ \\
        Open mean
        & Plan
        & $1.9\times$ & 0.32 & 0.60 & $\approx 0$ \\
        \midrule
        DSV4-F
        & Baseline
        & $15.6\times$ & 0.69 & 0.92 & $\approx 0$ \\
        DSV4-F
        & Plan
        & $5.2\times$ & 0.51 & 0.69 & $\approx 0$ \\
        \midrule
        DSV4-P
        & Baseline
        & $16.1\times$ & 0.61 & 0.66 & $\approx 0$ \\
        DSV4-P
        & Plan
        & $12.0\times$ & 0.61 & 0.84 & $\approx 0$ \\
        \bottomrule
    \end{tabular}
    \caption{
        Effect of explicit planning at $N=20$.
        Coverage statistics use fixed scoring and random order;
        value correlations are measured in the matched random-scoring
        condition.
    }
    \label{tab:planning}
\end{table}

Crucially, planning changes the \emph{spread} of computation, not its \emph{priorities}. Correlations between effort and point value remain near zero. Difficulty sensitivity likewise does not meaningfully improve. The model learns to divide its effort more evenly, but not to direct that effort toward questions with higher expected return.

This distinction matters. Uniformity can improve coverage, especially on longer exams, but equal spending is not the same as strategic spending. A useful allocation policy should respond to differences in value, difficulty, and expected solvability. The explicit-planning prompt does not induce such behavior.

\subsection{RQ4: What Are the Score Consequences?}
\label{sec:score_consequences}

The previous sections analyze the allocation mechanism directly. We now connect that mechanism to the resulting exam scores. Two comparisons are especially informative: changing the relationship between difficulty and value, and comparing the emergent allocation with a simple equal split.

\subsubsection{Aligned and Reversed Scoring Reprice Similar Behavior}
\label{sec:repricing}

Aligned and reversed scoring assign different values to the same questions. Under aligned scoring, difficult questions are worth more; under reversed scoring, easy questions are worth more. A value-aware model should respond by changing which questions it attempts or how much effort it assigns to them.

Instead, models generally score higher under reversed scoring, as shown in Table~\ref{tab:repricing}. The aligned-minus-reversed difference is negative for every model. This does not mean the models have discovered that easy questions are more profitable. Rather, they continue to solve many of the same questions under both schemes. Reversed scoring simply assigns more points to the easier questions that the model was already likely to answer.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{7pt}
    \begin{tabular}{lrrr}
        \toprule
        \textbf{Model}
        & \textbf{Aligned}
        & \textbf{Reversed}
        & $\boldsymbol{\Delta}$ \\
        \midrule
        QW-14  & 22.1 & 37.5 & $-15.4$ \\
        DQ-14  & 25.4 & 39.1 & $-13.7$ \\
        DSV4-F & 48.2 & 60.1 & $-11.8$ \\
        QW-8   & 15.4 & 26.5 & $-11.2$ \\
        DSV4-P & 48.4 & 57.5 & $-9.1$ \\
        DQ-7   & 11.2 & 17.1 & $-5.9$ \\
        \bottomrule
    \end{tabular}
    \caption{
        Mean score rate (\%) under aligned and reversed scoring,
        using matched exams with random order and the baseline prompt.
        $\Delta$ is aligned minus reversed.
    }
    \label{tab:repricing}
\end{table}

At $N=10$, the overlap between the sets of correctly answered questions under the two scoring schemes is approximately 0.86. The overlap between work sets is lower, at approximately 0.68, but changes in effort are only weakly aligned with changes in point value: the correlation is approximately 0.2, and only 55\% of effort shifts move in the direction favored by the new scoring rule.

The score difference is therefore best understood as a \emph{repricing} of a broadly similar behavior. Models do not substantially reorganize their allocation when the reward structure changes.

\subsubsection{Ordering Can Make the Same Policy Look Better or Worse}
\label{sec:order_score}

The interaction between scoring and question order further illustrates this point. Table~\ref{tab:order_scoring} reports DSV4-F results. The highest score occurs when easy questions are both valuable and placed first. In that setting, a position-greedy policy happens to align with the scoring objective.

The opposite combination---hard questions first under reversed scoring---is adversarial. The model spends early computation on questions that are both expensive and low-value. The large differences across cells therefore arise even though the underlying allocation policy remains largely unchanged.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{crrrr}
        \toprule
        & \multicolumn{2}{c}{\textbf{Aligned}}
        & \multicolumn{2}{c}{\textbf{Reversed}} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        $\boldsymbol{N}$
        & \textbf{Easy first}
        & \textbf{Hard first}
        & \textbf{Easy first}
        & \textbf{Hard first} \\
        \midrule
        10 & 47.4 & 44.3 & 77.9 & 55.9 \\
        20 & 32.9 & 36.4 & 64.2 & 48.4 \\
        \bottomrule
    \end{tabular}
    \caption{
        DSV4-F score rate (\%) under the baseline prompt.
        Reversed scoring with easy questions first is favorable to a
        position-greedy solver; reversed scoring with hard questions
        first is adversarial.
    }
    \label{tab:order_scoring}
\end{table}

This sensitivity to presentation order is a consequence of allocation failure. A strategic model should adapt its policy when the ordering and reward structure change. Instead, score often depends on whether a largely fixed sequential policy happens to encounter favorable questions early.

\subsubsection{Comparison with Uniform Allocation}
\label{sec:uniform}

We also compare the shared-budget run with a simple equal split. In the \emph{uniform per-question} condition, each question is solved independently with a budget of $B/N$ tokens.

This condition should not be treated as an oracle. Independent prompts remove cross-question interference in addition to enforcing equal allocation. It is nevertheless a useful reference for asking whether the model's emergent allocation provides a consistent advantage over a naive split.

The answer depends on exam length. At $N=5$, the shared-budget setting outperforms uniform allocation for four of seven models and gains 2.6 score points on average. At $N=10$, the comparison is nearly even. At $N=20$, every model performs worse under the shared budget, with an average difference of $-5.0$ points.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{7pt}
    \begin{tabular}{crr}
        \toprule
        $\boldsymbol{N}$
        & \textbf{Shared wins}
        & $\boldsymbol{\Delta}$ \\
        \midrule
        5  & 4/7 & $+2.6$ \\
        10 & 3/7 & $-0.4$ \\
        20 & 0/7 & $-5.0$ \\
        \bottomrule
    \end{tabular}
    \caption{
        Shared-budget performance relative to uniform per-question
        allocation under aligned scoring, random order, and the
        baseline prompt. $\Delta$ is the mean score-rate difference
        in percentage points: shared minus uniform.
    }
    \label{tab:uniform}
\end{table}

We therefore do not claim that shared-budget inference always loses to a uniform split. At small $N$, front-loading can occasionally help by allowing the model to complete a few questions with high confidence. The comparison becomes consistently unfavorable only as the exam grows and coverage collapses.

The mechanism-level conclusions do not depend on this reference. Regardless of whether the shared-budget score is above or below the uniform condition in a particular cell, the allocation remains dominated by prompt position and largely insensitive to point value.

\subsection{Cross-Domain Check: CRUXEval-O}
\label{sec:crux_results}

The preceding analyses use olympiad mathematics. We next ask whether the same pattern appears in a different reasoning domain. We use CRUXEval-O \citep{pmlr-v235-gu24c}, where the model is given a short Python function and an input and must predict the exact return value.

This experiment is intended as a targeted cross-domain check rather than a second full-factorial study. We construct 50 exams for each $N\in\{10,20\}$ and evaluate QW-14, DQ-14, DSV4-F, and DSV4-P. Because CRUXEval-O does not provide native difficulty labels, we use fixed and random scoring, random question order, and the baseline and explicit-planning prompts. Answers are evaluated using deterministic structured matching.

We set the shared reasoning budget to $B=3{,}000$ tokens. To make the constraint comparable with the mathematics setting, we estimate the typical unconstrained cost from high-budget independent runs on correctly answered items and approximately match
\begin{equation}
    \frac{B}{
        N \times
        \text{typical unconstrained cost per question}
    }
\end{equation}
across domains. The median unconstrained cost for CRUXEval-O is approximately 995 tokens per correctly answered question.

The code results closely reproduce the mathematical pattern. Averaged across models and exam lengths under the baseline prompt, token effort correlates with prompt position at $\rho=-0.42$, while solving order correlates at $\rho=0.99$. Under random scoring, the corresponding value correlations are only 0.02 for effort and $-0.04$ for solving order. The models therefore follow the prompt almost exactly while remaining insensitive to the stated point values.

Table~\ref{tab:crux_position} shows the per-model results. Coverage again deteriorates as the number of questions increases. At $N=20$, zero-token rates range from 30\% to 47\%, and 71\%--83\% of all reasoning tokens are spent on the first half of the prompt. Nearly all runs exhaust the available budget.

\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{4.5pt}
    \begin{tabular}{lcrrrrrrr}
        \toprule
        \textbf{Model}
        & $\boldsymbol{N}$
        & $\boldsymbol{\rho(\text{effort},\text{pos.})}$
        & $\boldsymbol{\rho(\text{order},\text{pos.})}$
        & $\boldsymbol{R_{\mathrm{FB}}}$
        & \textbf{Front share}
        & \textbf{Zero}
        & \textbf{Hit budget}
        & \textbf{Accuracy} \\
        \midrule
        QW-14
        & 10 & $-0.39^{*}$ & 1.00 & 1.76 & 63\% & 24\% & 88\% & 49.6\% \\
        QW-14
        & 20 & $-0.67^{*}$ & 1.00 & 5.22 & 83\% & 47\% & 98\% & 47.2\% \\
        \midrule
        DQ-14
        & 10 & $-0.16^{*}$ & 0.94 & 1.36 & 51\% & 23\% & 83\% & 39.8\% \\
        DQ-14
        & 20 & $-0.59^{*}$ & 1.00 & 3.89 & 76\% & 42\% & 100\% & 34.7\% \\
        \midrule
        DSV4-F
        & 10 & $-0.20^{*}$ & 0.97 & 1.47 & 57\% & 19\% & 70\% & 86.2\% \\
        DSV4-F
        & 20 & $-0.65^{*}$ & 1.00 & 4.07 & 79\% & 40\% & 100\% & 80.8\% \\
        \midrule
        DSV4-P
        & 10 & $-0.13^{*}$ & 0.98 & 1.10 & 51\% & 8\% & 56\% & 92.8\% \\
        DSV4-P
        & 20 & $-0.59^{*}$ & 1.00 & 2.68 & 71\% & 30\% & 96\% & 79.0\% \\
        \bottomrule
    \end{tabular}
    \caption{
        Allocation on CRUXEval-O under fixed scoring, random order,
        and the baseline prompt. Front share is the fraction of
        attributed tokens assigned to the first half of the exam.
        Asterisks indicate $p<0.05$.
    }
    \label{tab:crux_position}
\end{table*}

Accuracy separates the models far more than allocation does. The API models answer 79\%--93\% of items correctly, roughly twice the rate of QW-14 and DQ-14, yet their effort--position and order--position correlations are indistinguishable from those of the open models. Whatever the code-reasoning ability of the model, the shared budget is spent in the same sequential way.

Explicit planning again affects coverage more than prioritization. At $N=20$, it reduces the front/back ratio from 5.22 to 4.31 for QW-14, from 3.89 to 3.72 for DQ-14, and from 2.68 to 2.48 for DSV4-P. DSV4-F changes little. Across all four models, correlations between effort and point value remain between $-0.04$ and 0.07, and accuracy changes inconsistently.

CRUXEval-O therefore reproduces the same qualitative mechanism: models spend disproportionately on early questions, follow presentation order, ignore point values, and cover less of the exam as $N$ grows. Planning can flatten the distribution, but does not make it value-aware. The shared-budget allocation failure is thus not specific to olympiad mathematics.

==> sec/setup.tex <==
\section{Problem Setup: Shared-Budget Multi-Question Reasoning}
\label{sec:setup}

\subsection{Task formulation}
An exam instance is $\mathcal{E}=\{(q_i,s_i)\}_{i=1}^{N}$: question $q_i$ with point value $s_i$. The model receives all questions in one prompt and a single global reasoning budget $B$ output tokens. Its objective is to maximize $\sum_i s_i \cdot \mathbf{1}\{\text{correct}_i\}$ subject to using at most $B$ tokens in Phase~1 (reasoning), after which per-question answers are elicited in Phase~2 with guided decoding to extract the answer. We use $B{=}20{,}000$ for math and a pressure-matched $B{=}3{,}000$ for code. 
This is isomorphic to a knapsack with \emph{latent} item costs (\S\ref{sec:analysis}); here we define the operational protocol.

\subsection{Dataset and exam construction}
We sample $N$ problems from Omni-MATH~\cite{gao2024omnimathuniversalolympiadlevel} into 50 exam papers per ($N$, scoring, order, strategy) cell. Difficulty labels come from benchmark metadata but are not shown to the model. Mathematics provides verifiable answers, meaningful difficulty spread, and large per-question token-cost variance---a controlled first testbed for allocation behavior.

\paragraph{Code generality check.}
CRUXEval~\cite{pmlr-v235-gu24c} contains 800 short Python functions with input--output pairs. We use CRUXEval-O: given a function and input, predict the exact return value. We construct 50 papers per cell for $N{\in}\{10,20\}$. Because CRUXEval has no native per-item difficulty labels, we dropped the difficulty-conditioned scoring setting for evaluation on this dataset.

\subsection{Models}
We evaluate seven reasoning models at two scales; the short tag given in parentheses after each model is the abbreviation we use for it in all subsequent tables and figures. Five \textbf{mid-scale} models (7--32B) are served locally with vLLM~\citep{kwon2025vllm}: DeepSeek-R1-Distill-Qwen-7B and -14B (DQ-7, DQ-14)~\citep{guo2025deepseek}, and Qwen3-8B, -14B, and -32B (QW-8, QW-14, QW-32)~\citep{yang2025qwen3}. Two \textbf{frontier-scale} models, DeepSeek-V4 Flash and Pro (DSV4-F, DSV4-P), are accessed through the provider's API; per-question reasoning traces are recovered from the returned reasoning content. Because several models in both groups are open-weight, the distinction we draw throughout is one of scale and serving mode, not of weight availability. All models are sampled with $T{=}0.6$, top-$p{=}0.95$, and top-$k{=}20$.

% The mid-scale models cover the full math factorial grid, whereas DSV4-F/P cover the \texttt{align} grid plus the mechanism slices needed for every main math table, so both groups appear side by side in all math results. The CRUXEval-O check uses a four-model subset: QW-14, DQ-14, DSV4-F, and DSV4-P.

\subsection{Budget and inference protocol}
Phase~1 decoding is capped at $B$; on exhaustion we append an end-of-thinking token and query each \texttt{Q}$i$ separately in Phase~2. Math answers use \texttt{\textbackslash boxed\{\}} extraction and a GPT-5 LLM-as-judge (Appendix~\ref{append:Prompts}). CRUXEval-O answers are short Python literals and use a programmatic exact-match judge (Appendix~\ref{append:crux-judge}). \textbf{Token attribution} segments the reasoning trace by strict \texttt{Q}$n$:\ markers; per-question effort is the sum of attributed tokens. We use token-\emph{centroid} rank for solving order (not first mention) and define a \emph{work set} as questions with $\geq$200 tokens or $\geq$2 segments (Appendix).

\subsection{Experimental factors}
Table~\ref{tab:factor-summary} summarizes factors. We treat them as a factorial probe of allocation \emph{signals}, not a catalog of ablations. Each factor level below is introduced with the \texttt{typewriter} name we use to refer to it in all later sections, tables, and figures.

\paragraph{Score assignment (value axis).}
\texttt{fixed} (no value variance; clean position/difficulty tests), \texttt{random} (points $\perp$ difficulty \& position; clean value probe), \texttt{align} (hard = valuable; consequence setting), \texttt{reverse} (easy = valuable; punishes position-greedy solvers).

\paragraph{Question ordering.}
\texttt{orig} decouples difficulty from position within each paper; \texttt{asc}/\texttt{dsc} present easy-first or hard-first orderings.

\paragraph{Prompt strategies.}
\texttt{baseline} (default), \texttt{explicit\_plan} (intervention: plan budget before solving). Skip, recheck, and ALL variants are secondary (Appendix).

\paragraph{Reference lines (not oracles).}
\textbf{Unlimited per-Q} (40{,}960 tok/q, isolated): capability ceiling only. \textbf{Uniform per-Q} ($B/N$, isolated): naive equal split; confounds allocation with cross-question interference (stated upfront). For CRUXEval-O, the unlimited median is approximately 995 tokens per question, motivating $B{=}3{,}000\approx3\times$ median and matching the math pressure ratio at $N{=}10,20$.

\subsection{Metrics}
\textbf{Primary (mechanism):} per-question token effort; front/back ratio; zero-token and work-set coverage; Spearman/partial Spearman of effort and solving order vs.\ position, difficulty, points. CRUXEval-O reports position and points only because it lacks native difficulty labels.

\textbf{Secondary (consequence):} score rate; align$-$reverse tax; one-round minus uniform $\Delta$.

\input{img_tab_tex/tab_factor_summary}


==> sec/time.tex <==
\section{Timeline}

\begin{itemize}
    \item \textbf{Mar 6 - Mar 15: Proposal \& Baseline Setup.} Submit the initial proposal. Complete data preprocessing and establish the first-step deliverable by evaluating unconstrained baseline model performance.
    \item \textbf{Mar 16 - Mar 31: Core Experiments.} Evaluate difficulty-dependent scoring and question orderings (increasing, decreasing, random) under a fixed total budget.
    \item \textbf{Apr 1 - Apr 15: Strategy Evaluation \& Analysis.} Test explicit prompting strategies (e.g., planning and skipping). Finalize experiments and quantitatively analyze allocation behaviors.
    \item \textbf{Apr 16 - Apr 30: Report Drafting.} Draft the final project report, detailing the problem formulation, methodology, and empirical findings.
    \item \textbf{May 1 - May 11: Final Submission \& Poster Prep.} Submit the final report, design the poster, and prepare for the poster session.
\end{itemize}
